Bayesian Nonparametric Modeling of Driver Behavior using HDP Split-Merge Sampling Algorithm

Modern vehicles are equipped with increasingly complex sensors. These sensors generate large volumes of data that provide opportunities for modeling and analysis. Here, we are interested in exploiting this data to learn aspects of behaviors and the road network associated with individual drivers. Our dataset is collected on a standard vehicle used to commute to work and for personal trips. A Hidden Markov Model (HMM) trained on the GPS position and orientation data is utilized to compress the large amount of position information into a small amount of road segment states. Each state has a set of observations, i.e. car signals, associated with it that are quantized and modeled as draws from a Hierarchical Dirichlet Process (HDP). The inference for the topic distributions is carried out using HDP split-merge sampling algorithm. The topic distributions over joint quantized car signals characterize the driving situation in the respective road state. In a novel manner, we demonstrate how the sparsity of the personal road network of a driver in conjunction with a hierarchical topic model allows data driven predictions about destinations as well as likely road conditions.

==> hdpModel_2levelStick_paper.tex <==
\begin{tikzpicture}
  [latent/.style={circle,fill=white,draw=black,inner sep=3pt, minimum size=16pt, font=\fontsize{9}{9}\selectfont},
    obs/.style={latent,fill=gray!25},
  const/.style={rectangle,fill=gray!25, draw=black,inner sep=6pt,font=\fontsize{9}{9}\selectfont},
  invis/.style={circle,fill=white,draw=white}]
  \matrix[row sep=4mm,column sep=6mm, matrix anchor=mid] (lda) {
    & \\
    \node (alpha) [const] {$\alpha$}; & \node (pi) [latent] {$\pi_{d,i}$}; & \node (c) [latent] {$c_{d,i}$}; &\node (v) [latent] {$v_{k}$}; & \node (omega) [const] {$\omega$};  \\ 
                                       & \\
                                       &  \node (z) [latent] {$z_{d,n}$}; & \node (w) [obs]  {$w_{d,n}$}; &\node (beta) [latent] {$\beta_{k}$}; & \node (nu) [const] {$\nu$}; \\
                                       & \node (space) [invis] { $\,$ };& & & \\
  };

  %\node (alphalambda) [const, above=10pt of lambda]  {$\alpha_{\theta}$};
  %\node (alphaphi) [const, above=10pt of phi]  {$\alpha_{\phi}$};

  \draw [->] (alpha) -- (pi);
  \draw [->] (pi) -- (z);
  \draw [->] (z) -- (w);
  \draw [->] (omega) -- (v);
  \draw [->] (v) -- (c);
  \draw [->] (c) -- (w);
  \draw [->] (nu) -- (beta);
  \draw [->] (beta) -- (w);

  \plate{contentplatec}{(beta)(v)}{$\infty$}{inner sep=2pt, rounded corners=3,font=\fontsize{9}{9}}
  \plate{contentplatec}{(pi)(c)}{$\infty$}{inner sep=2pt, rounded corners=3,font=\fontsize{9}{9}}
  \plate{contentplatec}{(z)(w)}{$N_d$}{inner sep=2pt, rounded corners=3,font=\fontsize{9}{9}}
  \plate{contentplatec}{(pi)(c)(w)(z)(space)}{$D$}{inner sep=4pt, rounded corners=3,font=\fontsize{9}{9}}
\end{tikzpicture}


==> hdpModel_paper.tex <==
% Latent Dirichlet allocation
\begin{tikzpicture}
  [latent/.style={circle,fill=white,draw=black,inner sep=2pt, minimum size=18pt, font=\fontsize{12}{12}\selectfont},
    obs/.style={latent,fill=gray!25},
  const/.style={rectangle,fill=gray!25, draw=black,inner sep=2pt, minimum size=18pt,font=\fontsize{12}{12}\selectfont}]
  \matrix[row sep=2mm,column sep=10mm, matrix anchor=mid] (lda) {
    && \\
    && \\
    & & \node (base) [const] {$H(\nu)$}; \\
    && \\
    \node (omega) [const] {$\omega $}; && \node (G0) [latent] {$G_0$}; \\
                                      && \\
    \node (alpha) [const] {$\alpha$}; && \node (Gc) [latent] {$G_d$}; \\
                                      && \\
                                      && \node (beta) [latent]  {$\boldsymbol{\beta}_{d,n}$}; \\
                                      && \\
                                      && \node (xc) [obs]  {$w_{d,n}$}; \\
  };

  %\node (alphalambda) [const, above=10pt of lambda]  {$\alpha_{\beta}$};
  %\node (alphaphi) [const, above=10pt of phi]  {$\alpha_{\phi}$};

  \draw [->] (base) -- (G0);
  \draw [->] (omega) -- (G0);
  \draw [->] (G0) -- (Gc);
  \draw [->] (alpha) -- (Gc);
  \draw [->] (Gc) -- (beta);
  \draw [->] (beta) -- (xc);

  \plate{platei}{(beta)(xc)}{$n\in \left\{1,\dots,N_d \right\}$}{inner sep=2pt, rounded corners=3,font=\fontsize{12}{12}}
  \plate{platej}{(platei)(Gc)}{$d\in D$}{inner sep=2pt, rounded corners=3,font=\fontsize{12}{12}}
\end{tikzpicture}


==> hdpVarAndFull_paper.tex <==
\begin{tikzpicture}
  [latent/.style={circle,fill=white,draw=black,inner sep=2pt, minimum size=12pt, font=\fontsize{9}{9}\selectfont},
    obs/.style={latent,fill=gray!25},
  const/.style={rectangle,fill=gray!25, draw=black,rounded corners=2pt,inner sep=6pt,font=\fontsize{9}{9}\selectfont},
  invis/.style={circle,fill=white,draw=white}]
  \matrix[row sep=4mm,column sep=12mm, matrix anchor=mid] (lda) {
    & \\
    \node (alpha) [const] {$\alpha$}; & \node (pi) [latent] {$\pi_{d,i}$}; & \node (c) [latent] {$c_{d,i}$};& \node (space1) [invis] { $\,$ }; &\node (v) [latent] {$v_{k}$}; & \node (omega) [const] {$\omega$};  \\ 
                                       & \\
                                       &  \node (z) [latent] {$z_{d,n}$}; & \node (w) [obs]  {$w_{d,n}$}; &\node (space2) [invis] { $\,$ }; &\node (beta) [latent] {$\beta_{k}$}; & \node (nu) [const] {$\nu$}; \\
                                       & \node (space) [invis] { $\,$ };& & & \\
  };

  %\node (alphalambda) [const, above=10pt of lambda]  {$\alpha_{\theta}$};
  %\node (alphaphi) [const, above=10pt of phi]  {$\alpha_{\phi}$};

  \draw [->] (alpha) -- (pi);
  \draw [->] (pi) -- (z);
  \draw [->] (z) -- (w);
  \draw [->] (omega) -- (v);
  \draw [->] (v) -- (c);
  \draw [->] (c) -- (w);
  \draw [->] (nu) -- (beta);
  \draw [->] (beta) -- (w);

  \plate{contentplatec}{(beta)(v)}{\tiny{$\infty (\rightarrow K)$}}{inner sep=5pt,font=\fontsize{9}{9}}
  \plate{contentplatec}{(pi)(c) (space1)}{\tiny{$\infty (\rightarrow T)$}}{inner sep=2pt, font=\fontsize{9}{9}}
    \plate{contentplatec}{(z)(w)}{\tiny{$N_d$}}{inner sep=2pt,font=\fontsize{9}{9}}
    \plate{contentplatec}{(pi)(c)(w)(z)(space1)}{\tiny{$D$}}{inner sep=7pt, font=\fontsize{9}{9}}
\end{tikzpicture}


==> hdpVariational_paper.tex <==
\begin{tikzpicture}
  [latent/.style={circle,fill=white,draw=black,inner sep=3pt, minimum size=16pt, font=\fontsize{9}{9}\selectfont},
    obs/.style={latent,fill=gray!25},
  const/.style={rectangle,fill=gray!25, draw=black,inner sep=6pt,font=\fontsize{9}{9}\selectfont},
  invis/.style={circle,fill=white,draw=white}]
  \matrix[row sep=4mm,column sep=6mm, matrix anchor=mid] (lda) {
    & \\
    \node (alpha) [const] {$\alpha$}; & \node (pi) [latent] {$\pi_{d,i}$}; & \node (c) [latent] {$c_{d,i}$}; &\node (v) [latent] {$v_{k}$}; & \node (omega) [const] {$\omega$};  \\ 
                                       & \\
                                       &  \node (z) [latent] {$z_{d,n}$}; & \node (w) [obs]  {$w_{d,n}$}; &\node (beta) [latent] {$\beta_{k}$}; & \node (nu) [const] {$\nu$}; \\
                                       & \node (space) [invis] { $\,$ };& & & \\
  };

  %\node (alphalambda) [const, above=10pt of lambda]  {$\alpha_{\theta}$};
  %\node (alphaphi) [const, above=10pt of phi]  {$\alpha_{\phi}$};

  \draw [->] (alpha) -- (pi);
  \draw [->] (pi) -- (z);
  \draw [->] (z) -- (w);
  \draw [->] (omega) -- (v);
  \draw [->] (v) -- (c);
  \draw [->] (c) -- (w);
  \draw [->] (nu) -- (beta);
  \draw [->] (beta) -- (w);

  \plate{contentplatec}{(beta)(v)}{$K$}{inner sep=2pt, rounded corners=3,font=\fontsize{9}{9}}
  \plate{contentplatec}{(pi)(c)}{$T$}{inner sep=2pt, rounded corners=3,font=\fontsize{9}{9}}
  \plate{contentplatec}{(z)(w)}{$N_d$}{inner sep=2pt, rounded corners=3,font=\fontsize{9}{9}}
  \plate{contentplatec}{(pi)(c)(w)(z)(space)}{$D$}{inner sep=4pt, rounded corners=3,font=\fontsize{9}{9}}
\end{tikzpicture}


==> tkz-obj-marks.tex <==
% Copyright 2011 by Alain Matthes
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.


\def\fileversion{1.16 c}
\def\filedate{2011/06/01}


%<-------------------------------------------------------------------------–>
%                               Setup   Marks
%<-------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%                              DefSetOfPoints
%<--------------------------------------------------------------------------–>
\newif\iftkz@sop@show
\newcount\tkz@cntmk
\pgfkeys{
  /tkzSoPt/.cd,
  prefix/.code              = {\global\edef\tkz@pref{#1}},
  /tkzSoPt/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
                              \pgfkeysalso{\searchname/.try=#1,
                               /tikz/\searchname/.retry=#1}}  
}   
\def\tkzDefSetOfPoints{\pgfutil@ifnextchar[{\tkz@SetOfPoints}{%
                                         \tkz@SetOfPoints[]}}
\def\tkz@SetOfPoints[#1]#2{%
\begingroup 
\pgfkeys{%
/tkzSoPt/.cd,
prefix=tkzPt}
\pgfqkeys{/tkzSoPt}{#1} 
    \tkz@cntmk1 %
    \edef\tkz@@cnt{\the\tkz@cntmk}
    \foreach \x/\y in {#2}{% 
         \tkz@cntmk=\tkz@@cnt %
         \tkzDefPoint(\x,\y){\tkz@pref\the\tkz@cntmk}
         \advance\tkz@cntmk by1 % 
         \global\edef\tkz@@cnt{\the\tkz@cntmk}
    }%
\endgroup}%
%<-------------------------------------------------------------------------–> 
\pgfkeys{
  /tkzjoinmk/.cd,
  prefix/.code              = {\global\edef\tkz@pref{#1}},
  /tkzjoinmk/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
                              \pgfkeysalso{\searchname/.try=#1,
                               /tikz/\searchname/.retry=#1}}  
}  
\def\tkzJoinSetOfPoints{\pgfutil@ifnextchar[{\tkz@JoinSetOfPoints}{%
                                             \tkz@JoinSetOfPoints[]}} 
\def\tkz@JoinSetOfPoints[#1]{%
\begingroup
\pgfkeys{%
/tkzjoinmk/.cd,
prefix=tkzPt}
\pgfqkeys{/tkzjoinmk}{#1}  
\pgfmathsetcount{\tkz@cntmk}{\tkz@@cnt-2}
\edef\tkz@@cnt{\the\tkz@cntmk} 
\foreach \nb in {1,...,\tkz@@cnt}{%
\tkz@cntmk=\nb
\advance\tkz@cntmk by1 
\draw[line cap=round,/tkzjoinmk/.cd,#1] (\tkz@pref\nb)--(\tkz@pref\the\tkz@cntmk);}
\endgroup}   
%<-------------------------------------------------------------------------–>
%              ShowSetOfMark
%<-------------------------------------------------------------------------–>
\pgfkeys{
/tkzdrawmk/.cd,
prefix/.code                = {\global\edef\tkz@pref{#1}},
/tkzdrawmk/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
                              \pgfkeysalso{\searchname/.try=#1,
                               /tikz/\searchname/.retry=#1}}  
} 
\def\tkzDrawSetOfPoints{\pgfutil@ifnextchar[{\tkz@DrawSetOfPoints}{
                                             \tkz@DrawSetOfPoints[]}} 
\def\tkz@DrawSetOfPoints[#1]{%
\begingroup
\pgfkeys{/tkzdrawmk/.cd, prefix=tkzPt}
\pgfqkeys{/tkzdrawmk}{#1}  
\pgfmathsetcount{\tkz@cntmk}{\tkz@@cnt-1}  
\foreach \nb in {1,...,\tkz@cntmk}{%
\tkzDrawMark[#1](\tkz@pref\nb)}
\endgroup} 
 
%<-------------------------------------------------------------------------–>
%               tkzmark
%<-------------------------------------------------------------------------–>
\def\tkzDrawMark{\pgfutil@ifnextchar[{\tkz@DrawMark}{\tkz@DrawMark[]}}   
\def\tkz@DrawMark[#1](#2){%
    \draw plot[mark style,#1] coordinates {(#2)};  
}
%<-------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
\def\tkzDrawMarks{\pgfutil@ifnextchar[{\tkz@DrawMarks}{\tkz@DrawMarks[]}}  
\def\tkz@DrawMarks[#1](#2){%
\foreach \point in {#2}{%
\draw plot[mark style,#1] coordinates {(\point)}; % StyleMark,
}} 

%<--------------------------------------------------------------------------–>
%                Init pour mark
%<--------------------------------------------------------------------------–>
\pgfkeys{%
setupmk/.cd,
size/.code    =  {\global\edef\tkz@sum@mk@size{#1}},
color/.code   =  {\global\edef\tkz@sum@mk@color{#1}},
fill/.code    =  {\global\edef\tkz@sum@mk@fill{#1}}, 
mark/.code    =  {\global\edef\tkz@sum@mk@mark{#1}}
} 

\def\tkzSetUpMark{\pgfutil@ifnextchar[{\tkzActivOff\tkz@SetUpMark}{%
                                         \tkzActivOff\tkz@SetUpMark[]}} 

\def\tkz@SetUpMark[#1]{% 
 \pgfkeys{%
/setupmk/.cd,
mark    =  \tkz@mk@mark,
color   =  \tkz@mk@color,
fill    =  \tkz@mk@color!50,
size    =  \tkz@mk@size}
\pgfqkeys{/setupmk}{#1}
\tikzset{mark style/.style={inner sep    = 0pt,
                            mark         = \tkz@sum@mk@mark,
                            mark size    = \tkz@sum@mk@size,
                            mark options = {color = \tkz@sum@mk@color,
                                            fill  = \tkz@sum@mk@fill}}}
}%  

%<--------------------------------------------------------------------------–>
\endinput
  

==> tkz-obj-points.tex <==
% Copyright 2011 by Alain Matthes
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.


\def\fileversion{1.16 c}
\def\filedate{2011/06/01}


%<--------------------------------------------------------------------------–>
%                             init def point 
%<--------------------------------------------------------------------------–>
\newif\iftkz@polar\tkz@polarfalse
\newif\iftkz@pt@polar 
\newif\iftkz@pt@show 
\newif\iftkz@pt@noname

  
%<--------------------------------------------------------------------------–>
\pgfdeclareshape{cross}
{%
  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \foregroundpath{
% store lower right in xa/ya and upper right in xb/yb
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{0 pt}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{0 pt}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{0 pt}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{0 pt}}
 }
}
%<--------------------------------------------------------------------------–>
%                            tkzDefPoint
%<--------------------------------------------------------------------------–>

%<--------------------------------------------------------------------------–>
%                     macros complémentaires  pour def point
%<--------------------------------------------------------------------------–>
\def\tkz@parsecoordinate#1{%
\tkz@getseparator#1,\@nil
\iftkz@polar 
   \tkz@getfrompolar#1\@nil
\else
  \tkz@getfromcart#1\@nil
\fi
}
\def\tkz@getseparator#1,#2\@nil{%
\ifx\tkzempty#2\tkzempty%
   \tkz@polartrue
\else
   \tkz@polarfalse
\fi
}      
\def\tkz@getfrompolar#1:#2\@nil{
  \FPeval\tkz@a{(#1)}
  \FPeval\tkz@r{(#2)} 
\global\edef\tkz@polarrad{\tkz@r}
\global\edef\tkz@polarangle{\tkz@a}
} 
\def\tkz@getfromcart#1,#2\@nil{
  \FPeval\tkz@x{(#1)}
  \FPeval\tkz@y{(#2)}
\global\edef\tkz@absc{\tkz@x}
\global\edef\tkz@ord{\tkz@y}
}
%<--------------------------------------------------------------------------–>
% la macro defpoint les coordonnées cartésiennes ou polaires sont  traitées
% afin de pouvoir adaptées avec les unités choisies
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
\def\tkzDefPoint{\pgfutil@ifnextchar[{\tkzActivOff\tkz@DefPoint}{%
                                      \tkzActivOff\tkz@DefPoint[]}}

\def\tkz@DefPoint[#1](#2)#{% 
\tkz@parsecoordinate{#2}
\iftkz@polar
 \tkz@ptStar[polar](\tkz@polarangle,\tkz@polarrad){tkz@coord@temp}
 \else  
     \tkz@ptStar[](#2){tkz@coord@temp}
 \fi
\tkz@DefPointEnd[#1]}% 
\def\tkz@DefPointEnd[#1]#2{% 
 \coordinate[#1] (#2) at (tkz@coord@temp);
}
%<--------------------------------------------------------------------------–>
%                            tkzDefPoints
%<--------------------------------------------------------------------------–>
\def\tkzDefPoints{\pgfutil@ifnextchar[{\tkz@DefPoints}{%
                                       \tkz@DefPoints[]}}

\def\tkz@DefPoints[#1]#2{%
\begingroup
   \foreach \ptx/\pty/\name in {#2}{\tkzDefPoint[#1](\ptx,\pty){\name}}%
\endgroup
} %<--------------------------------------------------------------------------–>
%                Init pour Draw
%<--------------------------------------------------------------------------–>
\pgfkeys{%
setuppt/.cd,
size/.code    =  {\global\edef\tkz@pt@size{#1}},
color/.code   =  {\global\edef\tkz@pt@color{#1}},
fill/.code    =  {\global\edef\tkz@pt@fill{#1}}, 
shape/.code   =  {\global\edef\tkz@pt@shape{#1}}
} 
%<--------------------------------------------------------------------------–>
%                    tkzSetUpPoint  définit la forme d'un point
%<--------------------------------------------------------------------------–>
\def\tkzSetUpPoint{\pgfutil@ifnextchar[{\tkzActivOff\tkz@SetUpPoint}{%
                                         \tkzActivOff\tkz@SetUpPoint[]}}

\def\tkz@SetUpPoint[#1]{%
\pgfkeys{%
/setuppt/.cd,
size    =  \tkz@euc@pointsize,
color   =  \tkz@euc@pointcolor,
fill    =  \tkz@euc@pointcolor!50,
shape   =  \tkz@euc@pointshape}
\pgfqkeys{/setuppt}{#1}
\tikzset{point style/.style={draw         = \tkz@pt@color,
                             inner sep    = 0pt,
                             shape        = \tkz@pt@shape,
                             minimum size = \tkz@pt@size*\pgflinewidth,
                             fill         = \tkz@pt@fill}}}%
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%                       Draw Point   
%<--------------------------------------------------------------------------–> 
%<--------------------------------------------------------------------------–> 
%\tikzset{/drawpoint/size/.style={minimum size=#1*\pgflinewidth}}
\pgfkeys{/drawpoint/.cd, 
  size/.code    = {\tikzset{point style/.append style={%
                   minimum size = #1*\pgflinewidth}}},
  color/.code    = {\tikzset{point style/.append style={%
                   draw = #1}}}, 
  shape/.code    = {\tikzset{point style/.append style={%
                   shape=#1}}},
  fill/.code    = {\tikzset{point style/.append style={%
                   fill=#1}}}                                     }
    
\def\tkzDrawPoint{\pgfutil@ifnextchar[{\tkz@DrawPoint}{\tkz@DrawPoint[]}} 
\def\tkz@DrawPoint[#1](#2){%
\begingroup 
\pgfkeys{/drawpoint/.cd}
\pgfqkeys{/drawpoint}{#1}    
\node[point style] at (#2) {};
\endgroup
}

%<--------------------------------------------------------------------------–> 
\def\tkzDrawPoints{\pgfutil@ifnextchar[{\tkz@drawpts}{\tkz@drawpts[]}} 
%<--------------------------------------------------------------------------–> 
\def\tkz@drawpts[#1](#2){%
\begingroup
\pgfkeys{/drawpoint/.cd}
\pgfqkeys{/drawpoint}{#1}        
\foreach \point in {#2}{%
   \node[point style] at (\point) {};}
\endgroup 
}
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
% rename
%<--------------------------------------------------------------------------–>
% \def\tkzRenamePoint{\pgfutil@ifnextchar[{\tkzActivOff\tkz@RenamePoint}{%
%                                          \tkzActivOff\tkz@RenamePoint[]}}  
% \def\tkz@RenamePoint[#1](#2)#{%
% \coordinate (tkz@coord@temp) at (#2);%
% \pgfextractx{\pgf@x}{\pgfpointanchor{tkz@coord@temp}{center}}
% \pgfextracty{\pgf@y}{\pgfpointanchor{tkz@coord@temp}{center}}
% \tkz@ax\pgf@x %
% \tkz@ay\pgf@y %
% \tkz@RenamePointEnd[#1]}% 
%<--------------------------------------------------------------------------–>
\def\tkzRenamePoint(#1)#2{\coordinate (#2) at (#1);}
\def\tkz@RenamePointEnd[#1]#2{\coordinate[#1] (#2) at (\tkz@ax,\tkz@ay);}
\def\tkzGetPoint#1{\coordinate  (#1) at (tkzPointResult);} 
\def\tkzGetPoints#1#2{\coordinate  (#1) at (tkzFirstPointResult);%
                      \coordinate  (#2) at (tkzSecondPointResult);}
\def\tkzGetFirstPoint#1{\coordinate  (#1) at (tkzFirstPointResult);}
\def\tkzGetSecondPoint#1{\coordinate  (#1) at (tkzSecondPointResult);}
\def\tkzDefShiftPointCoord[#1](#2)#3{%
\begin{scope}[shift={(#1)}]
  \coordinate  (#3) at (#2);
\end{scope}
}%

\def\tkzDefShiftPoint[#1](#2)#3{%
 \tkz@@extractxy{#1}
 \tkz@ax\pgf@x %
 \tkz@ay\pgf@y %   
\begin{scope}[shift={(\tkz@ax,\tkz@ay)}]
   \coordinate  (#3) at (#2);
\end{scope}
}
%<-------------------------------------------------------------------------–>
%   tkzLabelPoint          Affichage des LABELS pour un point
%<-------------------------------------------------------------------------–> 
% \newif\iftkz@mode@show 
% \tikzoption{show}{\tikz@addmode{\tkz@mode@showfalse}}  
\tikzset{label style/.style={\tkz@euc@pointpos,\tkz@euc@labelcolor,font=\normalsize}}
\def\tkzLabelPoint{\pgfutil@ifnextchar[{\tkz@LabelPoint}{\tkz@LabelPoint[]}} 
\def\tkz@LabelPoint[#1](#2)#3{\node[label style,#1] at (#2) {#3};}%

\def\tkzLabelPoints{\pgfutil@ifnextchar[{\tkz@LabelPoints}{%
                                         \tkz@LabelPoints[]}}% 
\def\tkz@LabelPoints[#1](#2){%
 \foreach \point in {#2}{
 \node[label style,#1] at (\point) {$\point$};}
}%
%<--------------------------------------------------------------------------–>
%                                 Coord  
%<--------------------------------------------------------------------------–>
\newif\if@tkz@coord@noxdraw
\newif\if@tkz@coord@noydraw
\pgfkeys{
/tkzprcoord/.cd,
  xlabel/.code    = {\global\edef\tkz@xlabel{#1}},%
  ylabel/.code    = {\global\edef\tkz@ylabel{#1}}, 
  xstyle/.code    = {\tikzset{xcoord style/.append style={#1}}},
  ystyle/.code    = {\tikzset{ycoord style/.append style={#1}}},
  noxdraw/.is if    = @tkz@coord@noxdraw,
  noxdraw/.default  = true,
  noydraw/.is if    = @tkz@coord@noydraw,
  noydraw/.default  = true,    
 /tkzprcoord/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
                                 \pgfkeysalso{\searchname/.try=#1,
                                   /tikz/\searchname/.retry=#1}} 
}
                              \def\tkzPointShowCoord{\pgfutil@ifnextchar[{\tkz@PointShowCoord}{%
                                         \tkz@PointShowCoord[]}}     
\def\tkz@PointShowCoord[#1](#2){%
\begingroup 
\pgfkeys{%
tkzprcoord/.cd,
  xlabel  = {},
  ylabel  = {},
  xstyle  = {},
  ystyle  = {},
  noxdraw = false,
  noydraw   = false
  }
\pgfqkeys{/tkzprcoord}{#1} 
\if@tkz@coord@noxdraw\else\draw[arrow coord style] (#2)--(#2 |- tkz@xline); \fi 
\if@tkz@coord@noydraw\else \draw[arrow coord style] (#2)--(#2 -| tkz@yline);\fi   
\ifx\tkzutil@empty\tkz@xlabel
\else
  \protected@edef\tkz@temp{%  
  \noexpand\path (#2)--(#2 |- tkz@xline)
  \noexpand node[xcoord style]}\tkz@temp {\tkz@xlabel};
\fi
\ifx\tkzutil@empty\tkz@ylabel
\else
  \protected@edef\tkz@temp{%
  \noexpand\path (#2)--(#2 -| tkz@yline)
  \noexpand node[ycoord style]}\tkz@temp {\tkz@ylabel};
\fi    
\endgroup
}

%<-------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%                                       tkzPoint
%<--------------------------------------------------------------------------–>
\pgfkeys{
  tkzpt/.cd,  
  pos/.code          = {\def\tkz@pt@pos{#1}},
  size/.code         = {\def\tkz@pt@size{#1}},
  name/.code         = {\def\tkz@pt@name{#1}},
  namecolor/.code    = {\def\tkz@pt@namecolor{#1}},
  time/.code         = {\def\tkz@pt@time{#1}},
  color/.code        = {\def\tkz@pt@color{#1}},
  shape/.code        = {\def\tkz@pt@shape{#1}},
  polar/.is if       = tkz@pt@polar,
  polar/.default     = true,  
  noname/.is if      = tkz@pt@noname,
  noname/.default    = true
}

\def\tkz@node#1{\path[coordinate](\ptxa,\ptya) coordinate(#1);}  
\def\tkz@drawnode#1{\path[coordinate](\ptxa,\ptya) coordinate(#1);
\tkz@DrawPt{#1}
}

\def\tkz@draw@point#1{%
  \node[ inner sep    = 0pt,
         shape        = \tkz@pt@shape,%
         draw         = \tkz@pt@color,%
         minimum size = \tkz@pt@size*\pgflinewidth,%
         fill         = \tkz@pt@color] at (#1) {};}
          
\def\tkzPoint{\@ifstar\tkzptStar\tkzptNoStar}
\def\tkzptNoStar{\pgfutil@ifnextchar[{\tkz@ptNoStar}{\tkz@ptNoStar[]}} 
\def\tkz@ptNoStar[#1](#2,#3)#{%  
\pgfkeys{/tkzpt/.cd,
 noname    = false,%  pas de nom
 name      = {},%     le nom est vide 
 polar     = false,%
 namecolor = \tkz@euc@labelcolor,%  couleur du nom
 pos       = \tkz@euc@pointpos,% name
 shape     = \tkz@euc@pointshape,%
 color     = \tkz@euc@pointcolor,% couleur du point
 size      = \tkz@euc@pointsize,%
 time      = 0.5
} 
\pgfqkeys{/tkzpt}{#1}  
   \iftkz@pt@polar%
     \FPeval\tkz@x{(#2*cos(#3*\FPpi/180))}
     \FPeval\tkz@y{(#2*sin(#3*\FPpi/180))}
   \else
     \FPeval\tkz@x{(#2)}
     \FPeval\tkz@y{(#3)}
   \fi

 \FPadd{\ptxa}{\tkz@x}{-\tkz@init@xorigine}
 \FPadd{\ptya}{\tkz@y}{-\tkz@init@yorigine}
 \FPdiv{\ptxa}{\ptxa}{\tkz@init@xstep}
 \FPdiv{\ptya}{\ptya}{\tkz@init@ystep}
  \tkz@drawnode
}
% dessin du point (par défaut c'est un node donc il ne peut pas être scalé)
\def\tkz@DrawPt#1{%
  \iftkz@pt@noname%  pas de nom rien
  \else% si name={} alors on prend le nom du node sinon name
       \ifx\tkzutil@empty\tkz@pt@name\def\tkz@pt@name{$#1$}%
       \fi
       \protected@edef\tkz@temp{%
          \noexpand \node[\tkz@pt@pos]}\tkz@temp at (#1)%
          {\textcolor{\tkz@pt@namecolor} {\tkz@pt@name}};%    
  \fi
% on retrace ???  ici ou après le fi
\tkz@draw@point{#1}
}

%<--------------------------------------------------------------------------–>
%                                  Star version tkzPoint*   
%<--------------------------------------------------------------------------–>
\def\tkzptStar{\pgfutil@ifnextchar[{\tkz@ptStar}{\tkz@ptStar[]}} 
\def\tkz@ptStar[#1](#2,#3)#{%
\pgfkeys{/tkzpt/.cd,
 polar     = false,%
} 
\pgfqkeys{/tkzpt}{#1}  
\iftkz@pt@polar%
  \FPeval\tkz@x{(#3*cos(#2*\FPpi/180))}
  \FPeval\tkz@y{(#3*sin(#2*\FPpi/180))}
\else
  \FPeval\tkz@x{(#2)}
  \FPeval\tkz@y{(#3)}
\fi
\FPadd{\ptxa}{\tkz@x}{-\tkz@init@xorigine}
\FPadd{\ptya}{\tkz@y}{-\tkz@init@yorigine}
\FPdiv{\ptxa}{\ptxa}{\tkz@init@xstep}
\FPdiv{\ptya}{\ptya}{\tkz@init@ystep}
\tkz@node
}

%<--------------------------------------------------------------------------–>
%                                  Points   
%<--------------------------------------------------------------------------–>
\def\tkzPoints{\pgfutil@ifnextchar[{\tkz@Points}{\tkz@Points[]}}  
\def\tkz@Points[#1](#2){%
\begingroup
   \foreach \ptx/\pty/\name in {#2}{%
             \tkzPoint[#1](\ptx,\pty){\name}%
   }
\endgroup
}

   %<--------------------------------------------------------------------------–>
% macro d'affichage  % 
%<--------------------------------------------------------------------------–>
\pgfqkeys{/pointwith}
{ orthogonal/.code            =\def\tkz@numv{0},
  orthogonal normed/.code     =\def\tkz@numv{1},
  linear/.code                =\def\tkz@numv{2},
  linear normed/.code         =\def\tkz@numv{3},
  colinear/.code         args ={at #1} {\global\def\tkz@numv{4}
                                        \global\def\tkz@frompoint{#1}},
  K/.code                     =\def\tkz@Koeff{#1}
  } 

\def\tkzDefPointWith{\pgfutil@ifnextchar[{\tkz@DefPointWith}{%
           \tkz@DefPointWith[]}}
\def\tkz@DefPointWith[#1](#2){%
\pgfqkeys{/pointwith}{linear,K=1}
\pgfqkeys{/pointwith}{#1}
\ifcase\tkz@numv%
 % first case 0
   \tkz@VecKOrth[\tkz@Koeff](#2){tkzPointResult}
  \or% 1
   \tkz@VecKOrthNorm[\tkz@Koeff](#2){tkzPointResult}
  \or% 2
   \tkz@VecK[\tkz@Koeff](#2){tkzPointResult} 
  \or% 3
   \tkz@VecKNorm[\tkz@Koeff](#2){tkzPointResult}
  \or% 4
   \tkz@VecKCoLinear[\tkz@Koeff](#2,\tkz@frompoint){tkzPointResult} 
   \fi    
}

%<-------------------------------------------------------------------------–>
% % % Points aléatoires sur un segment, une droite, une demi-droite un cercle 
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%                          les points aléatoires
%<--------------------------------------------------------------------------–>
\def\tkz@numrp{0}
\pgfkeys{/tkzDefRandPoint/.cd,
rectangle/.code args={#1 and #2}{\global\def\tkz@numrp{0}%
                                 \global\def\tkz@infl{#1}%
                                 \global\def\tkz@supr{#2}},
segment/.code  args={#1--#2}{\global\def\tkz@numrp{1}%
                              \global\def\tkz@start{#1}%
                              \global\def\tkz@end{#2}}, 
line/.code args={#1--#2}{\global\def\tkz@numrp{2}%
                          \global\def\tkz@start{#1}%
                          \global\def\tkz@end{#2}},  
circle/.code args={center #1 radius #2}{\def\tkz@numrp{3}%
                                          \global\def\tkz@center{#1}
                                          \global\def\tkz@rad{#2}}
} 

\def\tkzGetRandPointOn{\pgfutil@ifnextchar[{\tkz@DefRandPointOn}{%
           \tkz@DefRandPointOn[]}}
\def\tkz@DefRandPointOn[#1]#2{% 
\begingroup
\pgfkeys{/tkzDefRandPoint/.cd}   
\pgfqkeys{/tkzDefRandPoint}{#1}  
\ifcase\tkz@numrp%
 % first case 0
 \tkzRandPointOnRect(\tkz@infl,\tkz@supr){#2}  
  \or% 1
 \tkzRandPointOnSegment(\tkz@start,\tkz@end){#2}  
  \or% 2
 \tkzRandPointOnLine(\tkz@start,\tkz@end){#2} 
  \or% 3
 \tkzRandPointOnCircle(\tkz@center,\tkz@rad){#2} 
\fi    
\endgroup
}

\def\tkzRandPointOnRect(#1,#2)#3{% 
\tkz@@extractxy{#1}
    \pgf@xa=\pgf@x\relax%
    \pgf@ya=\pgf@y\relax%   
\tkz@@extractxy{#2}
    \pgf@xb=\pgf@x\relax%
    \pgf@yb=\pgf@y\relax%     
\FPadd{\tkz@a}{\pgf@sys@tonumber{\pgf@xb}}{-\pgf@sys@tonumber{\pgf@xa}}
\FPadd{\tkz@b}{\pgf@sys@tonumber{\pgf@yb}}{-\pgf@sys@tonumber{\pgf@ya}}
  \pgfmathparse{rnd}\global\let\myrndone\pgfmathresult 
    \pgfmathparse{rnd}\global\let\myrndtwo\pgfmathresult  
\path[coordinate] ($(#1)+(\myrndone*\tkz@a pt,%
                          \myrndtwo*\tkz@b pt)$) coordinate (#3);
                          } 

\def\tkzRandPointOnSegment(#1,#2)#3{% 
  \pgfmathparse{rnd}\global\let\myrnd\pgfmathresult 
\path[coordinate]  ($ (#1)!\myrnd!(#2) $) coordinate (#3);} 

\def\tkzRandPointOnLine(#1,#2)#3{% 
  \pgfmathparse{rand}\global\let\myrnd\pgfmathresult 
\path[coordinate]  ($ (#1)!\myrnd!(#2) $) coordinate (#3);}

\def\tkzRandPointOnCircle(#1,#2)#3{% 
\pgfmathrandominteger{\myrnd}{0}{360}
\tkz@ax#2 %
\FPeval\tkz@xa{\pgf@sys@tonumber{\tkz@ax}*cos(\myrnd*\FPpi/180)} 
\FPeval\tkz@xb{\pgf@sys@tonumber{\tkz@ax}*sin(\myrnd*\FPpi/180)}  
\path[coordinate]($(#1) + (\tkz@xa pt,\tkz@xb pt) $) coordinate (#3);
}

%<--------------------------------------------------------------------------–>
%                    Coordonnées d'un point 
%    result in #2x et #2y    #1 est le point et on récupère ses coordonnées
% usage soit A un point \tkzGetPointCoord(A){V} alors \Vx = xA et \Vy = yA
% en cm 
% tkzGetPointCoord avec [#1] cm ou bien pt !!! %<--------------------------------------------------------------------------–>
\def\tkzGetPointCoord(#1)#2{%
\begingroup
\pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}
\pgfmathparse{\pgf@sys@tonumber{\pgf@x}/28.45274}
\global\let\tkzresultx\pgfmathresult
\global\expandafter\edef\csname #2x\endcsname{\tkzresultx}% 
\pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}}
\pgfmathparse{\pgf@sys@tonumber{\pgf@y}/28.45274}
\global\let\tkzresulty\pgfmathresult
\global\expandafter\edef\csname #2y\endcsname{\tkzresulty}
\endgroup
}  

\def\tkz@@extractxy#1{%
\pgfextractx{\pgf@x}{\pgfpointanchor{#1}{center}}
\pgfextracty{\pgf@y}{\pgfpointanchor{#1}{center}} 
}
\let\tkzGetPointxy\tkzGetPointCoord
%<--------------------------------------------------------------------------–>
  
\endinput


==> tkz-obj-segments.tex <==
% Copyright 2011 by Alain Matthes
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.


\def\fileversion{1.16 c}
\def\filedate{2011/06/01}  

%<--------------------------------------------------------------------------–>
%                               Setup   Segment
%<--------------------------------------------------------------------------–>

%<--------------------------------------------------------------------------–>
%                             draw      segment  (s)
%<--------------------------------------------------------------------------–>                              
\def\tkzDrawSegment{\pgfutil@ifnextchar[{\tkz@DrawSegment}{%
                                         \tkz@DrawSegment[]}} 
\def\tkz@DrawSegment[#1](#2,#3){%    
\begingroup
 \draw[line style,add=0 and 0,#1] (#2) to (#3); 
\endgroup   
}%    

\def\tkz@multiDrawSeg#1 #2\@nil{%
 \protected@edef\tkz@temp{
   \noexpand \tkzDrawSegment[\tkz@optseg](#1)}\tkz@temp%   
   \def\tkz@nextArg{#2}%
   \ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
   \fi
   \next#2\@nil
} 
\def\tkzDrawSegments{\pgfutil@ifnextchar[{\tkz@DrawSegments}{%
                                         \tkz@DrawSegments[]}}
\def\tkz@DrawSegments[#1](#2){% 
\global\edef\tkz@optseg{#1} 
\begingroup
   \let\next\tkz@multiDrawSeg
   \next#2 \@nil %    
\endgroup
}
%<-------------------------------------------------------------------------–> 
%<-------------------------------------------------------------------------–> 
\pgfkeys{tkzmarkoptions/.cd,
pos/.code        = {\global\def\tkz@mkpos{#1}},
color/.code      = {\global\def\tkz@mkcolor{#1}},
mark/.code       = {\global\def\tkz@mark{#1}},
size/.code       = {\global\def\tkz@mksize{#1}},
/tkzmarkoptions/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
                                \pgfkeysalso{\searchname/.try=#1,
                                 /tikz/\searchname/.retry=#1}
                                 } 
}  

\def\tkzMarkSegment{\pgfutil@ifnextchar[{\tkz@MarkSegment}{%
                                        \tkz@MarkSegment[]}}
\def\tkz@MarkSegment[#1](#2,#3){%
\pgfkeys{tkzmarkoptions/.cd,
         size   = 4pt,
         color  = \tkz@mk@color,
         pos    = .5,
         mark   = none}
\pgfqkeys{/tkzmarkoptions}{#1}

\global\def\tkz@mymark{%
  \pgfsetplotmarksize{\tkz@mksize}
  \pgfuseplotmark{\tkz@mark}
}
\begin{scope} [decoration={ markings,mark=at position \tkz@mkpos with \tkz@mymark}] 
\path [\tkz@mkcolor,postaction={decorate}] (#2) -- (#3);
\end{scope}
} 
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
% multiple
\def\tkz@multiMS#1 #2\@nil{%
 \protected@edef\tkz@temp{
   \noexpand \tkzMarkSegment[\tkz@optsg](#1)}\tkz@temp%
   \def\tkz@nextArg{#2}%
   \ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
   \fi
   \next#2\@nil
}
%<--------------------------------------------------------------------------–>
\def\tkzMarkSegments{\pgfutil@ifnextchar[{\tkz@MarkSegments}{%
                                          \tkz@MarkSegments[]}}
\def\tkz@MarkSegments[#1](#2){% 
\global\edef\tkz@optsg{#1} 
  \begingroup
   \let\next\tkz@multiMS
   \next#2 \@nil %    
\endgroup 
} 
%<--------------------------------------------------------------------------–>
%<------------------------- Label on segment -------------------------------–>
%<--------------------------------------------------------------------------–>
\def\tkzLabelSegment{\pgfutil@ifnextchar[{\tkz@LabelSegment}{%
                                        \tkz@LabelSegment[]}}
\def\tkz@LabelSegment[#1](#2,#3)#4{%
\begingroup    
\path  (#2) to node[above,#1]{#4} (#3) ;  
\endgroup 
} 
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
% multiple
\def\tkz@multiLS#1 #2\@nil{%
 \protected@edef\tkz@temp{
   \noexpand \tkzLabelSegment[\tkz@optls](#1){\tkz@labelseg}}\tkz@temp%
   \def\tkz@nextArg{#2}%
   \ifx\tkzutil@empty\tkz@nextArg
     \let\next\@gobble
   \fi
   \next#2\@nil
}
%<--------------------------------------------------------------------------–>
\def\tkzLabelSegments{\pgfutil@ifnextchar[{\tkz@LabelSegments}{%
                                           \tkz@LabelSegments[]}}
\def\tkz@LabelSegments[#1](#2)#3{% 
\global\edef\tkz@optls{#1}
\global\def\tkz@labelseg{#3}
  \begingroup
   \let\next\tkz@multiLS
   \next#2 \@nil %    
\endgroup 
} 
%<--------------------------------------------------------------------------–>
%                                 PolySeg
%<--------------------------------------------------------------------------–>
\def\tkzDrawPolySeg{\pgfutil@ifnextchar[{\tkz@DrawPolySeg}{%
                                         \tkz@DrawPolySeg[]}}
\def\tkz@DrawPolySeg[#1](#2,#3){% 
\begingroup
\draw[#1] (#2) 
    \foreach \tkz@pt in {#3}{--(\tkz@pt)};% 
\endgroup
}   
\endinput


==> tkz-tools-arith.tex <==
% Copyright 2011 by Alain Matthes
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.


\def\fileversion{1.161 c}
\def\filedate{2011/06/12}  
% 1.161  test if "isfactor"   is already defined

%<--------------------------------------------------------------------------–>
% Objet :  tools for arithmetic 
%<--------------------------------------------------------------------------–>
%    [About integers numbers]
%<--------------------------------------------------------------------------–>
\ProvidesFile{tkz-tool-arith.tex}[tkz-tool-arith 1.161 c]
\edef\tkzAtCode{\the\catcode`\@} 
\catcode`\@=11\relax
%<--------------------------------------------------------------------------–>
%                            arithmetic tools 
%<--------------------------------------------------------------------------–>

\tkzutil@ifundefined{pgfmath@function@gcd}{%
\pgfmathdeclarefunction{gcd}{2}{%
 \begingroup%
 \pgfmathcontinuelooptrue
    \pgfmath@xa=#1pt\relax%
    \pgfmath@xb=#2pt\relax%
    \ifdim\pgfmath@xa=0pt \pgfmathcontinueloopfalse
     \pgfmath@xa=\pgfmath@xb
    \fi 
     \ifdim\pgfmath@xb=0pt \pgfmathcontinueloopfalse
       \pgfmath@xb=\pgfmath@xa
    \fi
\loop
\ifpgfmathcontinueloop 
 \ifdim \pgfmath@xa=\pgfmath@xb\pgfmathcontinueloopfalse
 \else
  \ifdim \pgfmath@xa>\pgfmath@xb 
   \advance \pgfmath@xa by-\pgfmath@xb
  \else 
   \advance \pgfmath@xb by-\pgfmath@xa
  \fi
  \fi
  \repeat
  \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@xa}}%
  \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
}{} 
%<--------------------------------------------------------------------------->

\tkzutil@ifundefined{pgfmath@function@isprime}{%
\newif\ifpgf@unknown
\newif\ifpgf@isaprime    
\pgfmathdeclarefunction{isprime}{1}{%
	\begingroup%
\pgf@unknowntrue
\c@pgfmath@counta#1\relax% 
 \ifcase#1\relax 
 % |#1| = 0 
 \pgf@isaprimefalse\pgf@unknownfalse
 \or
 % |#1| = 1
  \pgf@isaprimefalse\pgf@unknownfalse
  \or
% |#1| = 2
  \pgf@isaprimetrue\pgf@unknownfalse
 \or
% |#1| = 3
  \pgf@isaprimetrue\pgf@unknownfalse
   \else
 % |#1| > 3
   \ifodd#1\relax 
   \else
    \pgf@isaprimefalse\pgf@unknownfalse
   \fi
 \fi  
\ifpgf@unknown
\c@pgfmath@countd=\thr@@ \pgf@isaprimetrue
 \loop
 \c@pgfmath@countb=\c@pgfmath@counta  
 \divide\c@pgfmath@countb by\c@pgfmath@countd
  \ifnum\c@pgfmath@countb>\c@pgfmath@countd \pgf@unknowntrue
  \else\pgf@unknownfalse\fi
    \multiply\c@pgfmath@countb by\c@pgfmath@countd
  \ifnum\c@pgfmath@countb=\c@pgfmath@counta  
   \global\pgf@isaprimefalse\pgf@unknownfalse\fi
  \ifpgf@unknown\advance\c@pgfmath@countd by 2\relax% 
 \repeat
\fi
\ifpgf@isaprime
  \def\pgfmathresult{1}%
\else
  \def\pgfmathresult{0}%
\fi
 \pgfmath@smuggleone\pgfmathresult%
\endgroup
}}{}  
%<--------------------------------------------------------------------------->
\tkzutil@ifundefined{pgfmath@function@isodd}{%   
\pgfmathdeclarefunction{isodd}{1}{%  
\begingroup
\ifodd #1 \def\pgfmathresult{1}%
\else\def\pgfmathresult{0}%
\fi
 \pgfmath@smuggleone\pgfmathresult%
\endgroup}
}{}  
%<--------------------------------------------------------------------------->
\tkzutil@ifundefined{pgfmath@function@isfactor}{%
   \pgfmathdeclarefunction{isfactor}{2}{%  
\begingroup 
\c@pgfmath@counta#1\relax%   
\c@pgfmath@countb#2\relax%   
\c@pgfmath@countc#1\relax%
\divide\c@pgfmath@counta by\c@pgfmath@countb%
\multiply\c@pgfmath@counta by\c@pgfmath@countb% 
\advance\c@pgfmath@countc by-\c@pgfmath@counta%
\ifnum\c@pgfmath@countc=0 \def\pgfmathresult{1}%
\else
  \def\pgfmathresult{0}%
  \fi
\pgfmath@smuggleone\pgfmathresult%
\endgroup} 
}{}  
%<--------------------------------------------------------------------------->
\def\tkzfactors#1{% 
\begingroup
\c@pgfmath@countb#1 
\pgfmathisprime{\c@pgfmath@countb}% 
\ifnum\pgfmathresult=1 
   \number\c@pgfmath@countb\ % prime number
\else% we can found factors
\tkz@factors{#1} 
\fi
\endgroup}% 
%<--------------------------------------------------------------------------–>
\def\tkz@factors#1{%
\begingroup
\c@pgfmath@countb#1 
\c@pgfmath@countd2\relax
 \loop
 \ifodd\c@pgfmath@countb\relax% 
 \else
  \divide\c@pgfmath@countb by2 %
   \number\c@pgfmath@countd\ % 
 \repeat%
%%%%%%%%%%%%%%
\def\tkzprim@last{1}%
\loop% first loop
  \ifnum\c@pgfmath@countb>1\relax
    \c@pgfmath@countd\tkzprim@last\relax
    \c@pgfmath@countc1\relax
%%%%%%%%%%%%%%
\tkz@find@last
%%%%%%%%%%%%%%
   \divide\c@pgfmath@countb by\c@pgfmath@countd\relax
   \number\c@pgfmath@countd\ %  affiche le facteur
\repeat% end first loop
%%%%%%%%%%%%%%   
\endgroup%
}%
%<--------------------------------------------------------------------------->
\def\tkz@find@last{%
     \ifnum\c@pgfmath@countc>\z@
     \edef\tkzprim@last{\the\c@pgfmath@countd}%
     \advance\c@pgfmath@countd by2\relax% begins with 3
     \c@pgfmath@counta\c@pgfmath@countb% macro mod !!
     \c@pgfmath@countc\c@pgfmath@counta%
     \divide\c@pgfmath@counta by\c@pgfmath@countd
     \multiply\c@pgfmath@counta by\c@pgfmath@countd
     \advance\c@pgfmath@countc by-\c@pgfmath@counta
      \let\tkz@find@next=\tkz@find@last
     \else
     \let\tkz@find@next=\relax%   
     \fi
     \tkz@find@next
}%
%<--------------------------------------------------------------------------->
%<--------------------------------------------------------------------------->
\def\tkzReducFrac#1#2{% 
\begingroup
\ifnum#1<0\relax%
   \c@pgfmath@counta=0\relax 
   \advance\c@pgfmath@counta by-#1
 \else
    \c@pgfmath@counta#1
 \fi
    \c@pgfmath@countb#2
    \pgfmathgcd{\c@pgfmath@counta}{\c@pgfmath@countb}%
    \pgfmathsetcount\c@pgfmath@countc{\pgfmathresult}
 \ifnum\c@pgfmath@counta=0\relax
   \c@pgfmath@counta#1
   \c@pgfmath@countb#2
 \else 
   \c@pgfmath@counta#1
   \c@pgfmath@countb#2
   \divide\c@pgfmath@counta by\c@pgfmath@countc%
   \divide\c@pgfmath@countb by\c@pgfmath@countc%
 \fi
\global\edef\tkzMathFirstResult{\the\c@pgfmath@counta}
\global\edef\tkzMathSecondResult{\the\c@pgfmath@countb} 
\endgroup}
%<--------------------------------------------------------------------------->
%<--------------------------------------------------------------------------->
%<--------------------------------------------------------------------------->

\catcode`\@=\tkzAtCode\relax 
\endinput




==> tkz-tools-base.tex <==
% tkz-tools-base.tex    
% Copyright 2011 by Alain Matthes
% This file may be distributed and/or modified
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.


%  utf8 encoding

\def\fileversion{1.16 c}
\def\filedate{2011/06/01}  

%<--------------------------------------------------------------------------–>
\global\let\@xa\tkz@init@xmin
\global\let\@xb\tkz@init@xmax
\global\let\@ya\tkz@init@ymin
\global\let\@yb\tkz@init@ymax 
%<--------------------------------------------------------------------------–>
\gdef\xgrad{1}
\gdef\ygrad{1}
\gdef\tkz@xa{0}
\gdef\tkz@xb{10}
\gdef\tkz@ya{0}
\gdef\tkz@yb{10}
\newif\iftkz@init@NO
\pgfkeys{
  /tkzInit/.cd,
  xmin/.code     = {\def\tkz@init@xmin{#1}},
  xmax/.code     = {\def\tkz@init@xmax{#1}},
  xstep/.code    = {\def\tkz@init@xstep{#1}},
  ymin/.code     = {\def\tkz@init@ymin{#1}},
  ymax/.code     = {\def\tkz@init@ymax{#1}},
  ystep/.code    = {\def\tkz@init@ystep{#1}}, 
  NO/.is if      = tkz@init@NO,
  NO/.default    = true   } 
  
\def\tkzInit{\pgfutil@ifnextchar[{\tkz@Init}{\tkz@Init[]}} 
\def\tkz@Init[#1]{%
\pgfkeys{/tkzInit/.cd,
         xmin  = 0,
         xmax  = 10,
         xstep = 1,
         ymin  = 0,
         ymax  = 10,
         ystep = 1,
         NO    = false 
}  
  \pgfqkeys{/tkzInit}{#1}
  \ifx\tkzfctloaded\undefined
    \else   
   \tkz@tkzf@fct=0 %  only if tkz-fct loaded
   \fi   
  \xdef\tkz@init@xorigine{0}
  \xdef\tkz@init@yorigine{0}
  \FPsgn\@xsgmin{\tkz@init@xmin}
  \FPsgn\@xsgmax{\tkz@init@xmax}
  \FPsgn\@ysgmin{\tkz@init@ymin}
  \FPsgn\@ysgmax{\tkz@init@ymax}
  \global\let\@xa\tkz@init@xmin
  \global\let\@xb\tkz@init@xmax
  \global\let\@ya\tkz@init@ymin
  \global\let\@yb\tkz@init@ymax
   \tkz@init@NOfalse  
  \ifx\@xsgmin\@xsgmax \tkz@init@NOtrue \fi
  \ifx\@ysgmin\@ysgmax \tkz@init@NOtrue  \fi
  \iftkz@init@NO%
  \ifx\@xsgmin\@xsgmax
    \FPadd{\tkz@init@xmax}{\tkz@init@xmax}{-\tkz@init@xmin}%
    \edef\tkz@init@xorigine{\tkz@init@xmin}
    \edef\tkz@init@xmin{0}
  \fi

  \ifx\@ysgmin\@ysgmax
    \FPadd{\tkz@init@ymax}{\tkz@init@ymax}{-\tkz@init@ymin}%
    \edef\tkz@init@yorigine{\tkz@init@ymin}
    \edef\tkz@init@ymin{0}
  \fi
  \fi
  \FPdiv{\tkz@xa}{\tkz@init@xmin}{\tkz@init@xstep}
  \FPdiv{\tkz@xb}{\tkz@init@xmax}{\tkz@init@xstep}
  \FPdiv{\tkz@ya}{\tkz@init@ymin}{\tkz@init@ystep}
  \FPdiv{\tkz@yb}{\tkz@init@ymax}{\tkz@init@ystep}
  \tkz@getdecimal{\tkz@init@xstep} % amélioration nb dec et integer
  \global\edef\tkz@init@xdec{\number\c@pgfmath@countb}
  \tkz@getdecimal{\tkz@init@ystep}
  \global\edef\tkz@init@ydec{\number\c@pgfmath@countb} 
}%
%<--------------------------------------------------------------------------–>
\pgfkeys{Clip/.cd, space/.code     = {\def\tkz@CLI@space{#1}}} 

\def\tkzClip{\pgfutil@ifnextchar[{\tkz@Clip}{\tkz@Clip[]}} 
\def\tkz@Clip[#1]{%
\pgfkeys{Clip/.cd,space    = {}} 
\pgfqkeys{/Clip}{#1} 
\ifx\tkzutil@empty\tkz@CLI@space
    \clip (\tkz@xa,\tkz@ya) rectangle (\tkz@xb,\tkz@yb);
 \else
    \FPadd{\tkz@xxa}{\tkz@xa}{-\tkz@CLI@space}
    \FPadd{\tkz@yya}{\tkz@ya}{-\tkz@CLI@space}
    \FPadd{\tkz@xxb}{\tkz@xb}{\tkz@CLI@space}
    \FPadd{\tkz@yyb}{\tkz@yb}{\tkz@CLI@space} 
    \clip (\tkz@xxa,\tkz@yya) rectangle (\tkz@xxb,\tkz@yyb);
\fi
} 
%todo add options
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–> 
\def\tkz@showgrad#1{%
\FPifint{#1}\FPtrunc\tkz@result{#1}{0}\else\FPset\tkz@result{#1}\fi}%

\def\tkz@Xresult{%
\tkz@showgrad{\xgrad}%
 $\numprint{\tkz@result}$%
}%
%<--------------------------------------------------------------------------–>
\def\tkz@Yresult{%
\tkz@showgrad{\ygrad}%
$\numprint{\tkz@result}$
}% 
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
\def\tkz@Xshowgradresult{% 
\iftkz@X@orig
\tkz@Xresult% 
\else % orig 
       \iftkz@init@NO% 
          \unless\ifx\tkz@pos\tkz@posmin
          \tkz@Xresult\fi
       \else % NO  
         \unless\ifx\tkz@pos\x@tkzero%
         \tkz@Xresult
         \fi%end of x@tkzero
      \fi%end of NO
\fi%end of orig
}%
%<--------------------------------------------------------------------------–>
\def\tkz@Yshowgradresult{% 
\iftkz@Y@orig
\tkz@Yresult%
\else % orig 
     \iftkz@init@NO%
        \unless\ifx\tkz@pos\tkz@posmin
        \tkz@Yresult\fi
      \else % NO
        \unless\ifx\tkz@pos\y@tkzero%
        \tkz@Yresult
       \fi%end of x@tkzero
    \fi%end of NO
\fi%end of orig
}%
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
\def\tkz@Xshowgrad{% 
\iftkz@X@orig
\tkzprintfrac% 
\else % orig 
       \iftkz@init@NO% 
          \unless\ifx\tz@pos\tkz@posmin
          \tkzprintfrac\fi
       \else % NO  
         \unless\ifx\tz@pos\x@tkzero%
         \tkzprintfrac
         \fi%end of x@tkzero
      \fi%end of NO
\fi%end of orig
}%
%<--------------------------------------------------------------------------–>
\def\tkz@Yshowgrad{% 
\iftkz@Y@orig
\tkzprintfrac%
\else % orig 
     \iftkz@init@NO%
        \unless\ifx\tz@pos\tkz@posmin
        \tkzprintfrac\fi
      \else % NO
        \unless\ifx\tz@pos\y@tkzero%
        \tkzprintfrac
       \fi%end of x@tkzero
    \fi%end of NO
\fi%end of orig
}%

%<--------------------------------------------------------------------------–>
%              Setup   axe
%<--------------------------------------------------------------------------–>
\pgfkeys{tkzaxis/.cd,
line width/.code         = {\global\edef\tkz@sua@lw{#1}},
color/.code              = {\global\edef\tkz@sua@color{#1}},
tickwd/.code             = {\global\edef\tkz@sua@tickwd{#1}},
ticka/.code              = {\global\edef\tkz@sua@ticka{#1}},
tickb/.code              = {\global\edef\tkz@sua@tickb{#1}}
} 

\def\tkzSetUpAxis{\pgfutil@ifnextchar[{\tkz@SetUpAxis}{\tkz@SetUpAxis[]}} 
\def\tkz@SetUpAxis[#1]{%
\begingroup
 \pgfkeys{/tkzaxis/.cd,
 line width  = \tkz@init@lw,
 color       = \tkz@init@color,
 tickwd      = \tkz@init@tickwd,
 ticka       = \tkz@init@ticka,
 tickb       = \tkz@init@tickb
 }
\pgfqkeys{/tkzaxis}{#1}
\global\let\tkz@init@lw\tkz@sua@lw
\global\let\tkz@init@gradsize\tkz@sua@gradsize 
\global\let\tkz@init@color\tkz@sua@color 
\global\let\tkz@init@tickwd\tkz@sua@tickwd 
\global\let\tkz@init@ticka\tkz@sua@ticka 
\global\let\tkz@init@tickb\tkz@sua@tickb  
\endgroup}
%<--------------------------------------------------------------------------–>
%                 tkzDrawX      todo améliorer les unités
%<--------------------------------------------------------------------------–>
\pgfkeys{%     prob avec space
tkzdrawX/.cd,
color/.code                = {\global\def\tkz@X@color{#1}},
label/.code                = {\global\def\tkz@X@label{#1}}, 
right space/.code          = {\global\def\tkz@axe@rxspace{#1}}, 
left space/.code           = {\global\def\tkz@axe@lxspace{#1}},
noticks/.is if             = tkz@X@noticks,
noticks/.default           = true, 
trig/.code                 = {\global\def\tkz@X@trig{#1}},    
step/.code                 = {\FPeval\tkz@posnext{#1}},  
tickwd/.code               = {\global\def\tkz@X@tickwd{#1}},
tickup/.code               = {\global\def\tkz@X@tickup{#1}},
tickdn/.code               = {\global\def\tkz@X@tickdn{#1}},   
/tkzdrawX/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
                              \pgfkeysalso{\searchname/.try=#1,
                               /tikz/\searchname/.retry=#1}}}
                                     
\def\tkzDrawX{\pgfutil@ifnextchar[{\tkz@DrawX}{\tkz@DrawX[]}}
\def\tkz@DrawX[#1]{
\begingroup%
\pgfkeys{/tkzdrawX/.cd,
color       = \tkz@init@color,
label       = \tkz@init@xlabel,
trig        = 0,
step        = \tkz@init@xstep,
right space = \tkz@init@rightspace,
left space  = \tkz@init@leftspace,
noticks     = false,
tickwd      = \tkz@init@tickwd,
tickup      = \tkz@init@ticka,
tickdn      = \tkz@init@tickb}
\pgfqkeys{/tkzdrawX}{#1}
\FPtrunc\tkz@posmax{\tkz@xb}{\tkz@init@xdec}
\FPtrunc\tkz@posmin{\tkz@xa}{\tkz@init@xdec}
\FPadd\tkz@xbsup{\tkz@xb}{\tkz@axe@rxspace}
\FPadd\tkz@xainf{\tkz@xa}{-\tkz@axe@lxspace}
\path (\tkz@xainf,0)--(\tkz@xbsup,0) node(tkz@xline){};
\draw[xaxe style,
      color = \tkz@X@color, 
      /tkzdrawX/.cd, #1] (\tkz@xainf,0)--(\tkz@xbsup,0)
      node[xlabel style, /tkzdrawX/.cd, #1]{\tkz@X@label};
 \iftkz@X@noticks
 \else 
  \ifnum\tkz@X@trig=0
   \FPtrunc\tkz@posmax{\tkz@posmax}{\tkz@init@xdec}%
   \FPdiv\tkz@posnext{\tkz@posnext}{\tkz@init@xstep}
   \FPadd\tz@posnext{\tkz@posmin}{\tkz@posnext}
   \foreach \tz@pos in {\tkz@posmin,\tz@posnext,...,\tkz@posmax}{% 
     \draw[color = \tkz@X@color,
           line width = \tkz@X@tickwd,
           shift      = {(\tz@pos,0)}]%
           (0pt,\tkz@X@tickup)--(0pt,-\tkz@X@tickdn);} 
    \else
       \FPadd{\tkz@posmin}{\tkz@posmin}{.5}% 
       \FPdiv\tkz@posmax{\tkz@posmax}{\FPpi}%
        \FPmul\tkz@posmax{\tkz@posmax}{\tkz@X@trig}% 
        \FPdiv\tkz@posmin{\tkz@posmin}{\FPpi}%
        \FPmul\tkz@posmin{\tkz@posmin}{\tkz@X@trig}%
        \FPround\tkz@posmin{\tkz@posmin}{0}% 
        \foreach \tz@pos in {\tkz@posmin,...,\tkz@posmax}{% 
           \FPmul\tz@pospi{\tz@pos}{\FPpi}
           \FPdiv\tz@pospi{\tz@pospi}{\tkz@X@trig}%
           \draw[color = \tkz@X@color,
                 line width = \tkz@X@tickwd,%
                 shift      = {(\tz@pospi,0)}]%
           (0pt,\tkz@X@tickup)--(0pt,-\tkz@X@tickdn);
         }% end foreach
         \fi
 \fi
\endgroup}
%<--------------------------------------------------------------------------–>
\pgfkeys{%     prob avec space
tkzAxeX/.cd,
color/.code                 = {\def\tkz@X@color{#1}},
label/.code                 = {\global\def\tkz@X@label{#1}},
frac/.code                  = {\def\tkzX@frac{#1}},
trig/.code                  = {\def\tkzX@trig{#1}},
/tkzAxeX/.unknown/.code     = {\let\searchname=\pgfkeyscurrentname
                               \pgfkeysalso{\searchname/.try=#1,
                               /tikz/\searchname/.retry=#1}}} 
                                
\def\tkzAxeX{\pgfutil@ifnextchar[{\tkz@AxeX}{\tkz@AxeX[]}}
\def\tkz@AxeX[#1]{%
\begingroup  
\tkzLabelX[#1] \tkzDrawX[#1] 
\endgroup
}


%<--------------------------------------------------------------------------–>
%                 tkzDrawY      todo améliorer les unités
%<--------------------------------------------------------------------------–>
\pgfkeys{%     prob avec space
tkzdrawY/.cd,
color/.code                = {\def\tkz@Y@color{#1}},
label/.code                = {\def\tkz@Y@label{#1}}, 
up space/.code             = {\global\def\tkz@axe@uyspace{#1}}, 
down space/.code           = {\global\def\tkz@axe@dyspace{#1}},
noticks/.is if             = tkz@Y@noticks,
noticks/.default           = true,
trig/.code                 = {\global\def\tkz@Y@trig{#1}},      
step/.code                 = {\FPeval\tkz@posnext{#1}},  
tickwd/.code               = {\global\def\tkz@Y@tickwd{#1}},
ticklt/.code               = {\global\def\tkz@Y@ticklt{#1}},
tickrt/.code               = {\global\def\tkz@Y@tickrt{#1}},   
/tkzdrawY/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
                              \pgfkeysalso{\searchname/.try=#1,
                               /tikz/\searchname/.retry=#1}}}
                                     
\def\tkzDrawY{\pgfutil@ifnextchar[{\tkz@DrawY}{\tkz@DrawY[]}}
\def\tkz@DrawY[#1]{%
\begingroup
\pgfkeys{/tkzdrawY/.cd,
color       = \tkz@init@color,
label       = \tkz@init@ylabel,
trig        = 0,
step        = \tkz@init@ystep,
up space    = \tkz@init@upspace,
down space  = \tkz@init@downspace,
noticks     = false,
tickwd      = \tkz@init@tickwd,
ticklt      = \tkz@init@tickb,
tickrt      = \tkz@init@ticka}
\pgfqkeys{/tkzdrawY}{#1}
\FPtrunc\tkz@posmax{\tkz@yb}{\tkz@init@ydec}
\FPtrunc\tkz@posmin{\tkz@ya}{\tkz@init@ydec}
\FPadd\tkz@ybsup{\tkz@yb}{\tkz@axe@uyspace}
\FPadd\tkz@yainf{\tkz@ya}{-\tkz@axe@dyspace}
\path (0,\tkz@yainf)--(0,\tkz@ybsup) node(tkz@yline){};
\draw[color = \tkz@Y@color,
      yaxe style,/tkzdrawY/.cd,#1] (0,\tkz@yainf)--(0,\tkz@ybsup)
      node[ylabel style,/tkzdrawY/.cd,#1]{\tkz@Y@label};
 \iftkz@Y@noticks
 \else 
   \ifnum\tkz@Y@trig=0   
   \FPtrunc\tkz@posmax{\tkz@posmax}{\tkz@init@ydec}%
   \FPdiv\tkz@posnext{\tkz@posnext}{\tkz@init@ystep}
   \FPadd\tz@posnext{\tkz@posmin}{\tkz@posnext}
   \foreach \tz@pos in {\tkz@posmin,\tz@posnext,...,\tkz@posmax}{% 
     \draw[color = \tkz@Y@color,
           line width = \tkz@Y@tickwd,
           shift       = {(0,\tz@pos)}]% 
            (\tkz@Y@tickrt,0pt)--(-\tkz@Y@ticklt,0pt);}
         \else
       \FPadd{\tkz@posmin}{\tkz@posmin}{.5}% 
       \FPdiv\tkz@posmax{\tkz@posmax}{\FPpi}%
        \FPmul\tkz@posmax{\tkz@posmax}{\tkz@Y@trig}% 
        \FPdiv\tkz@posmin{\tkz@posmin}{\FPpi}%
        \FPmul\tkz@posmin{\tkz@posmin}{\tkz@Y@trig}%
        \FPround\tkz@posmin{\tkz@posmin}{0}% 
        \foreach \tz@pos in {\tkz@posmin,...,\tkz@posmax}{% 
           \FPmul\tz@pospi{\tz@pos}{\FPpi}
           \FPdiv\tz@pospi{\tz@pospi}{\tkz@Y@trig}%
           \draw[color = \tkz@Y@color,
                line width = \tkz@Y@tickwd,%
                          shift      = {(0,\tz@pospi)}]%
           (\tkz@Y@tickrt,0pt)--(-\tkz@Y@ticklt,0pt);
         }% end foreach
         \fi     
 \fi        
\endgroup}
%<--------------------------------------------------------------------------->
\newif\iftkz@np 
\pgfkeys{%     prob avec space
tkzlabelX/.cd,
frac/.code                  = {\def\tkz@X@frac{#1}},
trig/.code                  = {\def\tkz@X@trig{#1}},  
step/.code                  = {\def\tkz@posnext{#1}},
label options/.code         = {\def\cmd@X@option{#1}},
np off/.is if               = tkz@np,
np off/.default             = true,
orig/.is if                 = tkz@X@orig,
orig/.default               = false,
tickwd/.code                = {\global\def\tkz@X@tickwd{#1}},
tickup/.code                = {\global\def\tkz@X@tickup{#1}},
tickdn/.code                = {\global\def\tkz@X@tickdn{#1}},   
/tkzlabelX/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
                              \pgfkeysalso{\searchname/.try=#1,
                               /tikz/\searchname/.retry=#1}}}  
                               \def\tkzLabelX{\pgfutil@ifnextchar[{\tkz@LabelX}{\tkz@LabelX[]}}
\def\tkz@LabelX[#1]{% 
\begingroup
\pgfkeys{/tkzlabelX/.cd,
frac          = 0,
trig          = 0,
step          = \tkz@init@xstep,
np off        = false,
orig          = true,
label options = {},
tickwd        = \tkz@init@tickwd,
tickup        = \tkz@init@ticka,
tickdn        = \tkz@init@tickb}  
\pgfqkeys{/tkzlabelX}{#1}
\iftkz@np\let\numprint@saved\numprint %
\let\numprint\relax\fi %    

\FPtrunc\tkz@posmin{\tkz@xa}{\tkz@init@xdec}% 
\FPtrunc\tkz@posmax{\tkz@xb}{\tkz@init@xdec}%
\FPtrunc\x@tkzero{0.0000000}{\tkz@init@xdec}% 

\ifnum\tkz@X@frac=0 %
  \ifnum\tkz@X@trig=0 % affichage normal
   \FPdiv\tz@posnext{\tkz@posnext}{\tkz@init@xstep}
   \FPadd\tz@posnext{\tkz@posmin}{\tz@posnext}      
   \foreach \tz@pos in {\tkz@posmin,\tz@posnext,...,\tkz@posmax}{%
     \FPtrunc\tkz@pos{\tz@pos}{\tkz@init@xdec}%
     \FPmul{\xgrad}{\tz@pos}{\tkz@init@xstep}%
     \FPadd{\xgrad}{\xgrad}{\tkz@init@xorigine}%
     \FPtrunc\xgrad{\xgrad}{\tkz@init@xdec}%
     \protected@edef\tkz@temp{%
     \noexpand\path[shift = {(\tz@pos,0)}]
     (0pt,\tkz@X@tickup)--(0pt,-\tkz@X@tickdn)%
     node[xlabel style,%
          fill = \tkz@fillcolor,
                 \cmd@X@option]}\tkz@temp{\tkz@Xshowgradresult}; 
}% 
  \else% trig > 0  
     \FPadd{\tkz@posmin}{\tkz@posmin}{.5}%
     \FPdiv\tkz@posmax{\tkz@posmax}{\FPpi}%
     \FPmul\tkz@posmax{\tkz@posmax}{\tkz@X@trig}% 
     \FPdiv\tkz@posmin{\tkz@posmin}{\FPpi}%
     \FPmul\tkz@posmin{\tkz@posmin}{\tkz@X@trig}%
     \FPround\tkz@posmin{\tkz@posmin}{0}% 
     \foreach \tz@pos in {\tkz@posmin,...,\tkz@posmax}{% 
        \tkzPrintFracWithPi{\tz@pos}{\tkz@X@trig}
        \FPmul\tz@pospi{\tz@pos}{\FPpi}
        \FPdiv\tz@pospi{\tz@pospi}{\tkz@X@trig}%
        \protected@edef\tkz@temp{%
        \noexpand\path[shift      = {(\tz@pospi,0)}]%
        (0pt,\tkz@X@tickup)--(0pt,-\tkz@X@tickdn)%
           node[xlabel style,
                text height = 8pt,
                fill        = \tkz@fillcolor,
                              \cmd@X@option]}\tkz@temp{\tkz@Xshowgrad};% 
      }% end foreach   
    \fi
\else% frac > 0  
\FPround\tkz@posmin{\tkz@posmin}{0}%  
   \foreach \tz@pos in {\tkz@posmin,...,\tkz@posmax}{%
    \tkzPrintFrac{\tz@pos}{\tkz@X@frac}% 
        \protected@edef\tkz@temp{%
        \noexpand\path[shift      = {(\tz@pos,0)}]%
          (0pt,\tkz@X@tickup)--(0pt,-\tkz@X@tickdn)%
          node[xlabel style,
               text height = 8pt,
               fill        = \tkz@fillcolor,
                             \cmd@X@option]}\tkz@temp{\tkz@Xshowgrad}%
   ;%    
  }% end foreach  
\fi
 \iftkz@np\let\numprint\numprint@saved \fi%      
\endgroup
} 

%<--------------------------------------------------------------------------->
\pgfkeys{%     prob avec space
tkzticksY/.cd,
frac/.code                  = {\def\tkz@Y@frac{#1}},
trig/.code                  = {\def\tkz@Y@trig{#1}},  
step/.code                  = {\def\tkz@posnext{#1}},
label options/.code         = {\def\cmd@Y@option{#1}}, 
np off/.is if               = tkz@np,
np off/.default             = true,
orig/.is if                 = tkz@Y@orig,
orig/.default               = false,
tickwd/.code               = {\global\def\tkz@Y@tickwd{#1}},
ticklt/.code               = {\global\def\tkz@Y@ticklt{#1}},
tickrt/.code               = {\global\def\tkz@Y@tickrt{#1}},      
/tkzticksY/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
                              \pgfkeysalso{\searchname/.try=#1,
                               /tikz/\searchname/.retry=#1}}}  
                               \def\tkzLabelY{\pgfutil@ifnextchar[{\tkz@LabelY}{\tkz@LabelY[]}}
\def\tkz@LabelY[#1]{%
\begingroup
\pgfkeys{/tkzticksY/.cd,
frac          = 0,
trig          = 0,
step          = \tkz@init@ystep,
np off        = false,  
orig          = true,  
label options = {},
tickwd        = \tkz@init@tickwd,
ticklt        = \tkz@init@tickb,
tickrt        = \tkz@init@ticka} 
\pgfqkeys{/tkzticksY}{#1}
\iftkz@np\let\numprint@saved\numprint %
\let\numprint\relax\fi % 

\FPtrunc\tkz@posmin{\tkz@ya}{\tkz@init@ydec}% 
\FPtrunc\tkz@posmax{\tkz@yb}{\tkz@init@ydec}%
\FPtrunc\y@tkzero{0.0000000}{\tkz@init@ydec}% 

\ifnum\tkz@Y@frac=0
  \ifnum\tkz@Y@trig=0 % affichage normal    
   \FPdiv\tz@posnext{\tkz@posnext}{\tkz@init@ystep}
   \FPadd\tz@posnext{\tkz@posmin}{\tz@posnext}      
   \foreach \tz@pos in {\tkz@posmin,\tz@posnext,...,\tkz@posmax}{%
     \FPtrunc\tkz@pos{\tz@pos}{\tkz@init@ydec}%
     \FPmul{\ygrad}{\tz@pos}{\tkz@init@ystep}%
     \FPadd{\ygrad}{\ygrad}{\tkz@init@yorigine}%
     \FPtrunc\ygrad{\ygrad}{\tkz@init@ydec}%
     \protected@edef\tkz@temp{%
     \noexpand\path[shift = {(0,\tz@pos)}]%
        (\tkz@Y@tickrt,0pt)--(-\tkz@Y@ticklt,0pt)%
        node[ylabel style, 
             fill  = \tkz@fillcolor,
                     \cmd@Y@option]}\tkz@temp{\tkz@Yshowgradresult};
}
  \else% trig > 0  
     \FPadd{\tkz@posmin}{\tkz@posmin}{.5}%
     \FPdiv\tkz@posmax{\tkz@posmax}{\FPpi}%
     \FPmul\tkz@posmax{\tkz@posmax}{\tkz@Y@trig}% 
     \FPdiv\tkz@posmin{\tkz@posmin}{\FPpi}%
     \FPmul\tkz@posmin{\tkz@posmin}{\tkz@Y@trig}%
     \FPround\tkz@posmin{\tkz@posmin}{0}% 
     \foreach \tz@pos in {\tkz@posmin,...,\tkz@posmax}{% 
        \tkzPrintFracWithPi{\tz@pos}{\tkz@Y@trig}
        \FPmul\tz@pospi{\tz@pos}{\FPpi}
        \FPdiv\tz@pospi{\tz@pospi}{\tkz@Y@trig}%
        \protected@edef\tkz@temp{%
        \noexpand\path[shift      = {(0,\tz@pospi)}]%
             (\tkz@Y@tickrt,0pt)--(-\tkz@Y@ticklt,0pt)%
             node[ylabel style,
                  text height  = 8pt,
                  fill         = \tkz@fillcolor,
                  \cmd@Y@option]}\tkz@temp{\tkz@Yshowgrad};% 
      }% end foreach   
    \fi    
\else% frac > 0  
\FPround\tkz@posmin{\tkz@posmin}{0}%
  \foreach \tz@pos in {\tkz@posmin,...,\tkz@posmax}{%
    \tkzPrintFrac{\tz@pos}{\tkz@Y@frac}% 
        \protected@edef\tkz@temp{%
        \noexpand\path[shift      = {(0,\tz@pos)}]%
          (\tkz@Y@tickrt,0pt)--(-\tkz@Y@ticklt,0pt)%
          node[ylabel style,
               text height   = 8pt,
               fill          = \tkz@fillcolor,
                               \cmd@Y@option]}\tkz@temp{\tkz@Yshowgrad}%
   ;% 
  }% end foreach
\fi
 \iftkz@np\let\numprint\numprint@saved \fi%      
\endgroup} 
%<--------------------------------------------------------------------------–>
\def\tkzAxeY{\pgfutil@ifnextchar[{\tkz@AxeY}{\tkz@AxeY[]}}
\def\tkz@AxeY[#1]{%
\begingroup
 \tkzDrawY[#1] \tkzLabelY[#1]   
\endgroup}
%<-------------------------------------------------------------------------->
\newif\if@tkz@swap
\pgfkeys{%     prob avec space
  tkzAxeXY/.cd,
  swap/.is if     = @tkz@swap,
  swap/.default   = true,
  /tkzAxeXY/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
                              \pgfkeysalso{\searchname/.try=#1,
                               /tikz/\searchname/.retry=#1}}}  
  
\def\tkzAxeXY{\pgfutil@ifnextchar[{\tkzAxe@XY}{\tkzAxe@XY[]}}  
\def\tkzAxe@XY[#1]{%
\pgfkeys{
  /tkzAxeXY/.cd,
  swap        = false}
\pgfqkeys{/tkzAxeXY}{#1}   
\if@tkz@swap
\tkzLabelX[#1]\tkzLabelY[#1]\tkzDrawX[#1]\tkzDrawY[#1]
\else
\tkzDrawX[#1]\tkzDrawY[#1]\tkzLabelX[#1]\tkzLabelY[#1]
\fi}
\def\tkzDrawXY{\pgfutil@ifnextchar[{\tkzDraw@XY}{\tkzDraw@XY[]}} 
\def\tkzDraw@XY[#1]{\tkzDrawX[#1]\tkzDrawY[#1]} 
\def\tkzLabelXY{\pgfutil@ifnextchar[{\tkzLabel@XY}{\tkzLabel@XY[]}}
\def\tkzLabel@XY[#1]{\tkzLabelX[#1]\tkzLabelY[#1]}     
%<--------------------------------------------------------------------------–>
%                                grid
%<--------------------------------------------------------------------------–>
\newif\if@tkz@gd@sub 
\def\tkzRatioLineGrid{0.75} 
\def\tkz@gd@sublw{0.4 pt} 


\pgfkeys{
  /tkzGrid/.cd,
  color/.code      = {\def\tkz@gd@color{#1}%
                      \edef\tkz@gd@subcolor{%
                      \tkz@gd@color!\tkzCoeffSubColor}},
  subxstep/.code   = {\def\tkz@gd@subxstep{#1}},
  subystep/.code   = {\def\tkz@gd@subystep{#1}},
    ratio/.code   = {\def\tkz@gd@ratio{#1}},
  line width/.code = {\edef\tkz@gd@lw{#1}
                      \edef\tkz@gd@sublw{\tkz@gd@ratio\tkz@gd@lw}},
  sub/.is if       = @tkz@gd@sub,
  sub/.default     = true ,
    /tkzGrid/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
                              \pgfkeysalso{\searchname/.try=#1,
                               /tikz/\searchname/.retry=#1}}} 
                               
\def\tkzGrid{\pgfutil@ifnextchar[{\tkz@Grid}{\tkz@Grid[]}}
\def\tkz@Grid[#1]{\@ifnextchar({\tkz@@Grid[#1]}%
                               {\tkz@@Grid[#1](\@xa,\@ya)(\@xb,\@yb)}}
\def\tkz@@Grid[#1](#2,#3)(#4,#5){%
\pgfkeys{
  /tkzGrid/.cd,
  sub        = false,
  color      = \tkz@grid@color,
  ratio    = 0.75, 
  subxstep   = \tkz@grid@xstep,
  subystep   = \tkz@grid@ystep,
  line width = \tkz@grid@lw}
  \pgfqkeys{/tkzGrid}{#1}   
    \begingroup
    \FPadd{\tkz@gxa}{#2}{-\tkz@init@xorigine}
    \FPadd{\tkz@gxb}{#4}{-\tkz@init@xorigine}
    \FPadd{\tkz@gya}{#3}{-\tkz@init@yorigine}
    \FPadd{\tkz@gyb}{#5}{-\tkz@init@yorigine}
    \FPdiv{\tkz@gxa}{\tkz@gxa}{\tkz@init@xstep}
    \FPdiv{\tkz@gya}{\tkz@gya}{\tkz@init@ystep}
    \FPdiv{\tkz@gxb}{\tkz@gxb}{\tkz@init@xstep}
    \FPdiv{\tkz@gyb}{\tkz@gyb}{\tkz@init@ystep}
    \if@tkz@gd@sub% 
      \FPeval\@subxstep{\tkz@gd@subxstep/\tkz@init@xstep}%
      \FPeval\@subystep{\tkz@gd@subystep/\tkz@init@ystep}%
      \draw [xstep      = \@subxstep cm,%
             ystep      = \@subystep cm,%
             color      = \tkz@gd@subcolor,%
             line width = \tkzRatioLineGrid]%
             (\tkz@gxa,\tkz@gya) grid (\tkz@gxb,\tkz@gyb);%
    \fi
    \draw [color      = \tkz@gd@color,%
           line width = \tkz@gd@lw]%
           (\tkz@gxa,\tkz@gya) grid (\tkz@gxb,\tkz@gyb);%
    \endgroup
}%
%<--------------------------------------------------------------------------–>
%                                repère
%<--------------------------------------------------------------------------–>

\newif\iftkz@Rep@orig
\pgfkeys{
  /tkzRep/.cd,
  line width/.code = {\def\tkz@Rep@lw{#1}},
  xlabel/.code     = {\def\tkz@Rep@xlabel{#1}},
  ylabel/.code     = {\def\tkz@Rep@ylabel{#1}},
  posxlabel/.code  = {\def\tkz@Rep@posxlabel{#1}},
  posylabel/.code  = {\def\tkz@Rep@posylabel{#1}},
  xnorm/.code      = {\def\tkz@Rep@xnorm{#1}}, 
  ynorm/.code      = {\def\tkz@Rep@ynorm{#1}},
  color/.code      = {\def\tkz@Rep@color{#1}},
  colorlabel/.code = {\def\tkz@Rep@colorlabel{#1}}}
  % /tkzRep/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
  %                             \pgfkeysalso{\searchname/.try=#1,
  %                              /tikz/\searchname/.retry=#1}}}   
%<--------------------------------------------------------------------------–>
\def\tkzRep{\pgfutil@ifnextchar[{\tkz@Rep}{%
                                 \tkz@Rep[]}} 
\def\tkz@Rep[#1]{%
\pgfkeys{
 /tkzRep/.cd, 
line width         = \tkz@sur@lw,
xlabel      = $\vec{\imath}$,
ylabel      = $\vec{\jmath}$,
posxlabel   = {\tkz@sur@posxlabel}, 
posylabel   = {\tkz@sur@posylabel},
xnorm       = 1,
ynorm       = 1,
color       = \tkz@sur@color,% remove ?
colorlabel  = \tkz@sur@colorlabel}% remove ? 
\pgfqkeys{/tkzRep}{#1} 
\begingroup
  \protected@edef\tkz@temp{%  
  \noexpand\draw [line width=\tkz@Rep@lw,color=\tkz@Rep@color,rep style]%
  (0,0) to node[\tkz@Rep@posylabel,color = \tkz@Rep@colorlabel]}\tkz@temp%
      {\tkz@Rep@ylabel}(0,\tkz@Rep@ynorm);
  \protected@edef\tkz@temp{%
  \noexpand \draw [line width=\tkz@Rep@lw,color=\tkz@Rep@color,rep style]%
   (0,0) to  node[\tkz@Rep@posxlabel,color = \tkz@Rep@colorlabel]}\tkz@temp%
      {\tkz@Rep@xlabel}(\tkz@Rep@xnorm,0);  
\endgroup 
} 
\def\tkzAddName{\pgfutil@ifnextchar[{\tkz@AddName}{\tkz@AddName[]}} 
\def\tkz@AddName[#1]#2{%
\node[above left,#1] at (\pgf@path@lastx,\pgf@path@lasty){#2};  
}% 
\endinput

==> tkz-tools-math.tex <==
% Copyright 2011 by Alain Matthes
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.


\def\fileversion{1.16 c}
\def\filedate{2011/06/01}  



% Objet :  outils mathématiques pour la géométrie euclideienne avec pgf/tikz
% utilisable de préférence avec un repère orthonormé et le cm comme unité 
% utile pour la compatibilité avec pgf 2
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%             Duplicate Length      à revoir pas de pt pas de global
% ||v(CN)||= ||v(AB)|| et v(CN) colineaire à v(CD) 
% A-->#1 B-->#2 C-->#3 D-->#4 N-->#5   ?????
%<--------------------------------------------------------------------------–>
\def\tkzDuplicateLen(#1,#2)(#3,#4){%
\begingroup 
    \tkzCalcLength(#1,#2)\tkzGetLength{tkz@firstlen}% 
    \tkzCalcLength(#3,#4)\tkzGetLength{tkz@secondlen}%
    \FPdiv\tkz@ratio{\tkz@firstlen}{\tkz@secondlen}%
    \tkz@VecKCoLinear[\tkz@ratio](#3,#4,#3){tkzPointResult}%
\endgroup 
}
\let\tkzDuplicateSegment\tkzDuplicateLen     %<--------------------------------------------------------------------------–>
%                    Coordonnées d'un vecteur  (couple de points)  
% Deux points A et B donc un vecteur on récupère les coordonnées de v(AB)
% en cm 
% tkzGetVecCoord en cm ou en pt ???
%<--------------------------------------------------------------------------–>
%result in #3x et #3y #1 et #2 sont les points  
% passage en cm avec fp ? 
\def\tkzGetVectxy(#1,#2)#3{%
\begingroup 
\pgfpointdiff{\pgfpointanchor{#1}{center}}%
             {\pgfpointanchor{#2}{center}}%
\pgfmathparse{\pgf@sys@tonumber{\pgf@x}/28.45274}%
\global\let\tkzresultx\pgfmathresult
\pgfmathparse{\pgf@sys@tonumber{\pgf@y}/28.45274}%
\global\let\tkzresulty\pgfmathresult
\global\expandafter\edef\csname #3x\endcsname{\tkzresultx}% 
\global\expandafter\edef\csname #3y\endcsname{\tkzresulty}% 
\endgroup
}
\let\tkzGetVecCoord\tkzGetVectxy
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
\def\tkz@numv{0}
\pgfkeys{/tkzdefv/.cd,
K/.code      = {\pgfmathparse{#1}\global\def\tkz@ratio{\pgfmathresult}},
colinear/.code     args = {at #1}{\global\def\tkz@numv{0}%
                                  \global\def\tkz@frompoint{#1}},
orthogonal/.code        = {\global\def\tkz@numv{1}},
linear/.code            = {\global\def\tkz@numv{2}}\pgfmathparse{#1},
normed orthogonal/.code = {\global\def\tkz@numv{3}},
normed linear/.code     = {\global\def\tkz@numv{4}},
} 
\def\tkzDefVector[#1](#2,#3)#4{%
\begingroup 
\pgfkeys{/tkzdefv/.cd,K=1}
\pgfqkeys{/tkzdefv}{#1}
\ifcase\tkz@numv%
 % first case 0
 \tkzDefVectorfrom[\tkz@ratio](#2,#3){#4}
  \or% 1
  \tkz@VecKOrth[\tkz@ratio](#2,#3){#4} 
  \or% 2
  \tkz@VecK[\tkz@ratio](#2,#3){#4}
  \or% 3
  \tkz@VecKOrthNorm[\tkz@ratio](#2,#3){#4}
  \or% 4
  \tkz@VecKCoLinear[#1](#2,#3)#4
  \fi    
\endgroup
} 

\def\tkzDefVectorfrom[#1](#2,#3)#4{%    
\begingroup    
    \pgfpointdiff{\pgfpointanchor{#2}{center}}%
                 {\pgfpointanchor{#3}{center}}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
     \path[coordinate](\tkz@frompoint)--+(\tkz@ratio\pgf@xa,%
                                          \tkz@ratio\pgf@ya) coordinate (#4);
\endgroup
} 
%<--------------------------------------------------------------------------–>
%         VecKCoLinear  CN = K x AB  #1 pt #2 pt #3 pt #4 nb #5 pt result   
% il faut modifier cette macro : on supprime #3 pour la colinéarité
% Il suffit d'utiliser Replicate ou Duplicate     coeff dans #1
% v(CD)=#1 x v(AB) #1 le coeff; #2-->A #3-->B #4-->C  #5-->N
%<--------------------------------------------------------------------------–>
\def\tkzVecKCoLinear{\pgfutil@ifnextchar[{\tkz@VecKCoLinear}{\tkz@VecKCoLinear[1]}} 
\def\tkz@VecKCoLinear[#1](#2,#3,#4)#5{% 
\begingroup
   \pgfpointdiff{\pgfpointanchor{#2}{center}}%
                {\pgfpointanchor{#3}{center}}%
   \pgf@xa=\pgf@x%
   \pgf@ya=\pgf@y% 
   \pgfmathparse{#1}\edef\tkz@coeff{\pgfmathresult}
   \path[coordinate](#4)--+(\tkz@coeff\pgf@xa,\tkz@coeff\pgf@ya)%
          coordinate (#5);%  
\endgroup
}%  
%<--------------------------------------------------------------------------–>
%         v(AN)=#1 x v(AB)     
%   #1 le coeff; #2--> A #3--> B   #4-->N  tq    #4-#2 = #1*(#3-#2)                                 
%<--------------------------------------------------------------------------–>
\pgfkeys{
  /tkzscalev/.cd,
  ratio/.code      = {\pgfmathparse{#1}\global\edef\tkz@ratio{\pgfmathresult}}
  }  
\def\tkzScaleVector{\pgfutil@ifnextchar[{\tkz@ScaleVector}{%
                                         \tkz@ScaleVector[]}} 
\def\tkz@ScaleVector[#1](#2,#3)#4{% 
\begingroup
\pgfkeys{/tkzscalev/.cd,ratio=-1}
\pgfqkeys{/tkzscalev}{#1}  
   \pgfpointdiff{\pgfpointanchor{#2}{center}}%
                {\pgfpointanchor{#3}{center}}%
   \pgf@xa=\pgf@x%
   \pgf@ya=\pgf@y% 
    \path[coordinate](#2)--++(\pgf@xa *\tkz@ratio,\pgf@ya *\tkz@ratio)%
          coordinate (#4);%   
\endgroup
}%          
%<--------------------------------------------------------------------------–>
%                 Outils pour les vecteurs
%<--------------------------------------------------------------------------–>
%  ce sont des outils élémentaires qui à partir de deux points en définissent 
% un troisième 
% #1 si c'est une option alors c'est un nombre réel
% #2 et #3 sont deux points
% #4 est le nom du point qui résulte de la transformation
% exemple : \tkzVecKNorm (A,B){C} définit un point C tel que AC = 1 et C est %  %  un point de la droite (AC). #1 peut être négatif

%<--------------------------------------------------------------------------–>
%              VectorNormalised ou K*VectorNormalised
% A-->#2 B-->#3 N-->#4      v(AB)  devient v(AN) tq ||v(AN)||=1 si #1=1  
%  sinon ||v(AN)||=#1 
%<--------------------------------------------------------------------------–>
\def\tkzVecKNorm{\pgfutil@ifnextchar[{\tkz@VecKNorm}{\tkz@VecKNorm[1]}} 
\def\tkz@VecKNorm[#1](#2,#3)#4{%
\begingroup
    \tkzpointnormalised{%
    \pgfpointdiff{\pgfpointanchor{#2}{center}}
                 {\pgfpointanchor{#3}{center}}}
    \pgf@xa=\pgf@x\relax%
    \pgf@ya=\pgf@y\relax% 
    \pgfmathparse{#1}\edef\tkz@coeff{\pgfmathresult}
    \FPmul\tkz@coeff{28.45274}{\tkz@coeff}
    \FPmul\tkz@x{\tkz@coeff}{\pgf@sys@tonumber{\pgf@xa}}
    \FPmul\tkz@y{\tkz@coeff}{\pgf@sys@tonumber{\pgf@ya}}
    \path[coordinate](#2)--++(\tkz@x pt,\tkz@y pt)%
          coordinate (#4);%
\endgroup
}%
%<--------------------------------------------------------------------------–>
%         v(AN)=#1 x v(AB)     
%   #1 le coeff; #2--> A #3--> B   #4-->N  tq    #4-#2 = #1*(#3-#2)                                 
%<--------------------------------------------------------------------------–>
\def\tkzVecK{\pgfutil@ifnextchar[{\tkz@VecK}{\tkz@VecK[1]}} 
\def\tkz@VecK[#1](#2,#3)#4{% 
\begingroup 
   \pgfpointdiff{\pgfpointanchor{#2}{center}}%
                {\pgfpointanchor{#3}{center}}%
   \pgf@xa=\pgf@x%
   \pgf@ya=\pgf@y% 
   \pgfmathparse{#1}\edef\tkz@coeff{\pgfmathresult}
    \path[coordinate](#2)--++(\pgf@xa *\tkz@coeff,%
                              \pgf@ya *\tkz@coeff)%
          coordinate (#4);%   
\endgroup
}% 
%<--------------------------------------------------------------------------–>
%                   tkzVector K Orth   coeff dans #1
%    v(AN) perp v(AB)  v(AB) v(AN) sens direct cercle trigo 
% ||v(AN)||=||v(AB)||
%<--------------------------------------------------------------------------–>
\def\tkzVecKOrth{\pgfutil@ifnextchar[{\tkz@VecKOrth}{\tkz@VecKOrth[1]}}  
\def\tkz@VecKOrth[#1](#2,#3)#4{%
\begingroup
    \pgfpointdiff{\pgfpointanchor{#2}{center}}%
                 {\pgfpointanchor{#3}{center}}%
    \pgf@xa=-\pgf@y%
    \pgf@ya=\pgf@x%
    \pgfmathparse{#1}\edef\tkz@coeff{\pgfmathresult}
    \path[coordinate](#2)--++(\tkz@coeff\pgf@xa,\tkz@coeff\pgf@ya)%
          coordinate (#4);%
\endgroup
}% 
%<--------------------------------------------------------------------------–>
%              tkzVecKOrthNorm   coeff dans #1
%    v(AN) perp v(AB)  v(AB) v(AN) sens direct cercle trigo 
% ||v(AN||=1 si #1 est vide ou =1 sinon ||v(AN||=K
%<--------------------------------------------------------------------------–>
\def\tkzVecKOrthNorm{\pgfutil@ifnextchar[{\tkz@VecKOrthNorm}%
                                         {\tkz@VecKOrthNorm[1]}}
\def\tkz@VecKOrthNorm[#1](#2,#3)#4{%    
\begingroup
 \tkzpointnormalised{\pgfpointdiff{\pgfpointanchor{#2}{center}}%
                                  {\pgfpointanchor{#3}{center}}} 
  \pgf@xa=-\pgf@y%
  \pgf@ya=\pgf@x%
  \FPmul\tkz@coeff{28.45274}{#1}
  \FPmul\tkz@x{\tkz@coeff}{\pgf@sys@tonumber{\pgf@xa}}
  \FPmul\tkz@y{\tkz@coeff}{\pgf@sys@tonumber{\pgf@ya}}
  \path[coordinate](#2)--++(\tkz@x pt,\tkz@y pt)%
          coordinate (#4);%    
\endgroup
}%      
%<--------------------------------------------------------------------------–>
%  \tkzpointnormalised    normalise un point A-->A' tq ||v(OA')=1||
% équivalent de \pgfpointnormalised avec fp
% example
% \tkzpointnormalised{%
% \pgfpointdiff{\pgfpointanchor{A}{center}}
%              {\pgfpointanchor{B}{center}}}

% or
% \pgf@x=1 cm
% \pgf@y=12 cm 
% \tkzpointnormalised{} %<--------------------------------------------------------------------------–> 
\def\tkzpointnormalised#1{%
\pgf@process{#1}%
\FPmul{\tkz@sx}{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@x}}
\FPmul{\tkz@sy}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@y}}
\FPadd{\tkz@sxy}{\tkz@sx}{\tkz@sy}
\FProot{\tkz@den}{\tkz@sxy}{2}
\FPdiv{\tkz@coordx}{\pgf@sys@tonumber{\pgf@x}}{\tkz@den}
\FPround{\tkz@coordx}{\tkz@coordx}{5}
\FPdiv{\tkz@coordy}{\pgf@sys@tonumber{\pgf@y}}{\tkz@den}
\FPround{\tkz@coordy}{\tkz@coordy}{5}
\pgf@x = \tkz@coordx pt
\pgf@y = \tkz@coordy pt
}
%<--------------------------------------------------------------------------–>
% restaure and save length
\def\tkz@save@length{%
\global\let\tkz@temp@length\tkzLengthResult}%
\def\tkz@restore@length{%
 \global\let\tkzLengthResult\tkz@temp@length }% 
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
%    \tkzCalcLength      Distance entre deux points en pt ou en cm  avec FP 
% \veclen mais avec fp 
%  option cm le résultat est en cm sinon en pt
%<--------------------------------------------------------------------------–>

\newif\iftkzLengthIncm
\pgfkeys{
DefVecLen/.cd,
       cm/.is if         = tkzLengthIncm,
       cm/.default       = true}   

\def\tkzCalcLength{\pgfutil@ifnextchar[{\tkz@CalcLength}{\tkz@CalcLength[]}}  
\def\tkz@CalcLength[#1](#2,#3){%
\pgfkeys{DefVecLen/.cd, cm = false}
\pgfqkeys{/DefVecLen}{#1}%   
\begingroup
\tkz@@CalcLength(#2,#3){tkzLengthResult}
\iftkzLengthIncm  
    \FPdiv\tkzFPMathLen{\tkzFPMathLen}{28.45274}
   \FPround\tkzFPMathLen\tkzFPMathLen5\relax% 
   \global\let\tkzLengthResult\tkzFPMathLen  
\fi 
\endgroup
}%
\def\tkz@@CalcLength(#1,#2)#3{%
\pgfpointdiff{\pgfpointanchor{#1}{center}}%
             {\pgfpointanchor{#2}{center}}%
\pgf@xa=\pgf@x%
\pgf@ya=\pgf@y%
\FPeval\tkz@temp@a{\pgfmath@tonumber{\pgf@xa}}%
\FPeval\tkz@temp@b{\pgfmath@tonumber{\pgf@ya}}%
\FPeval\tkz@temp@sum{(\tkz@temp@a*\tkz@temp@a+\tkz@temp@b*\tkz@temp@b)}%
\FProot{\tkzFPMathLen}{\tkz@temp@sum}{2}%
\FPround\tkzFPMathLen\tkzFPMathLen5\relax
\global\expandafter\edef\csname #3\endcsname{\tkzFPMathLen}
}
%<--------------------------------------------------------------------------–>
\def\tkzGetLength#1{%
\global\expandafter\edef\csname #1\endcsname{\tkzLengthResult}}  
%<--------------------------------------------------------------------------–>
%     \tkzpttocm  passage de pt à cm div par 28.45274
%<--------------------------------------------------------------------------–>
\def\tkzpttocm(#1)#2{%
\begingroup  
    \FPdiv\tkz@mathresult{#1}{28.45274}
    \FPround\tkz@mathresult\tkz@mathresult5\relax%  
     \global\let\tkz@mathresult\tkz@mathresult
     \global\expandafter\edef\csname #2\endcsname{\tkz@mathresult}% 
\endgroup
}%
%<--------------------------------------------------------------------------–>
%     \tkzcmtopt  passage de cm à pt mul par 28.45274  %<--------------------------------------------------------------------------–
\def\tkzcmtopt(#1)#2{%
\begingroup 
    \FPmul\tkz@mathresult{#1}{28.45274}
    \FPround\tkz@mathresult\tkz@mathresult5\relax%  
     \global\let\tkz@mathresult\tkz@mathresult
\global\expandafter\edef\csname #2\endcsname{\tkz@mathresult}% 
\endgroup  
}% 
%<--------------------------------------------------------------------------–>
%                          Slope
%<--------------------------------------------------------------------------–>
\def\tkzFindSlope{\tkz@FindSlope}
\def\tkz@FindSlope(#1,#2)#3{%
    \begingroup
 \tkzpointnormalised{\pgfpointdiff{\pgfpointanchor{#1}{center}}%
                                  {\pgfpointanchor{#2}{center}}}    
    \tkz@ax=\pgf@x\relax%
    \tkz@ay=\pgf@y\relax%
    \FPdiv{\tkz@Slope}{\pgfmath@tonumber{\tkz@ay}}{\pgfmath@tonumber{\tkz@ax}}
    \FPround{\tkz@Slope}{\tkz@Slope}{5}
    \global\expandafter\edef\csname #3\endcsname{\tkz@Slope}%  
\endgroup
}
%<--------------------------------------------------------------------------–>
%<----------------– for compatibility --------------------------------------–>
%<--------------------------------------------------------------------------–>
\def\tkzmathanglebetweenpoints#1#2{%
\begingroup
  \pgf@process{\pgfpointdiff{#1}{#2}}%
  %
  % First approximate the angle of the external point...
  %
  \pgf@xa\pgf@x%
  \pgf@ya\pgf@y%
  \pgf@xb\pgf@x%
  \pgf@yb\pgf@y%
  \ifdim\pgf@xa<0pt\relax%
    \pgf@xa-\pgf@xa%
  \fi
  \ifdim\pgf@ya<0pt\relax%
    \pgf@ya-\pgf@ya%
  \fi
  \ifdim\pgf@ya>\pgf@xa%
    \pgf@x\pgf@xa%
    \pgf@y\pgf@ya%
  \else
    \pgf@x\pgf@ya%
    \pgf@y\pgf@xa%
  \fi
  \ifdim\pgf@y=0pt\relax%
    \pgf@x0pt%
  \else 
  \FPdiv\pgfmathresult{1}{\pgfmath@tonumber{\pgf@y}}
  \FPround\pgfmathresult\pgfmathresult5\relax% 
    \pgf@x\pgfmathresult\pgf@x%
  \fi
  \multiply\pgf@x1000\relax%
  \afterassignment\pgfmath@gobbletilpgfmath@%
  \expandafter\c@pgf@counta\the\pgf@x\relax\pgfmath@%
\expandafter\pgf@x\csname pgfmath@atan@\the\c@pgf@counta\endcsname pt\relax%
    \ifdim\pgfmath@ya>\pgfmath@xa\relax%
      \pgf@x-\pgf@x%
      \advance\pgf@x90pt%
    \fi
    \ifdim\pgf@xb<0pt%
      \ifdim\pgf@yb>0pt%
        \pgf@x-\pgf@x%
      \fi
      \advance\pgf@x180pt\relax%
    \else
      \ifdim\pgf@yb<0pt%
      \pgf@x-\pgf@x%
      \advance\pgf@x360pt\relax%
    \fi 
    \fi
    \ifdim\pgf@x>180pt%
    \advance\pgf@x-360pt\relax%
    \fi
    \pgfmath@returnone\pgf@x%
  \endgroup
}

% \tkzmathrotatepointaround
%
% Rotate point #1 about point #2 by #3 degrees.
%
\def\tkzmathrotatepointaround#1#2#3{%
  \pgf@process{%
    \pgf@process{#1}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgf@process{#2}%
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \pgf@xb\pgf@x%
    \pgf@yb\pgf@y%
    \pgf@x=\pgf@xc%
    \pgf@y=\pgf@yc%
    \advance\pgf@x-\pgf@xa%
    \advance\pgf@y-\pgf@ya%
    \pgfmathsetmacro\tkz@angle{#3}%
    \pgfmathsin@{\tkz@angle}%
    \let\sineangle\pgfmathresult%
    \pgfmathcos@{\tkz@angle}%
    \let\cosineangle\pgfmathresult%
    \pgf@xa\cosineangle\pgf@x%
    \advance\pgf@xa-\sineangle\pgf@y%
    \pgf@ya\sineangle\pgf@x%
    \advance\pgf@ya\cosineangle\pgf@y%
    \pgf@x\pgf@xb%
    \pgf@y\pgf@yb%
    \advance\pgf@x\pgf@xa%
    \advance\pgf@y\pgf@ya%
  }%
}


% \tkzmathanglebetweenlines
%
% Calculate the clockwise angle between a line from point #1
% to point #2 and a line from #3 to point #4.
%
\def\tkzmathanglebetweenlines#1#2#3#4{%
  \begingroup
    \tkzmathanglebetweenpoints{#1}{#2}%
    \let\firstangle\pgfmathresult%
    \tkzmathanglebetweenpoints{#3}{#4}%
    \let\secondangle\pgfmathresult%
    \ifdim\firstangle pt>\secondangle pt\relax%
      \pgfmathadd@{\secondangle}{360}%
      \let\secondangle\pgfmathresult%
    \fi
    \pgfmathsubtract@{\secondangle}{\firstangle}%
    \pgfmath@smuggleone\pgfmathresult%
  \endgroup
} 
% \pgfmathpointreflectalongaxis
%
% Reflects point #2 around an axis centered on #2 at an angle #3.
%
\def\tkzmathreflectpointalongaxis#1#2#3{%
  \pgf@process{%
    \pgfmathanglebetweenpoints{#2}{#1}%
    \pgfmath@tempdima\pgfmathresult pt\relax%
    \pgfmathparse{#3}%
    \advance\pgfmath@tempdima-\pgfmathresult pt\relax%
    \pgfmath@tempdima-2.0\pgfmath@tempdima%
    \pgfmathrotatepointaround{#1}{#2}{\pgfmath@tonumber{\pgfmath@tempdima}}%
  }%
}


% \pgfmathpointintersectionoflineandarc 
%
% A bit experimental at the moment:
%
% Locates the point where a line crosses an eliptical arc. If the line
% does not cross the arc, a meaningless point will result.
%
% #1 the point of the line on the "convex" side of the arc.
% #2 the point of the line on the "concave" side of the arc.
% #3 the center of the eliptical arc.
% #4 start angle of the arc.
% #5 end angle of the arc.
% #6 radii of the arc.
%
\def\tkzmathpointintersectionoflineandarc#1#2#3#4#5#6{%
  \pgf@process{%
    %
    % Get the required angle.
    %
    \pgfmathanglebetweenpoints{#2}{#1}%
    \let\x\pgfmathresult%
    %
    % Get the radii of the arc.
    %
    \pgfmath@in@{and }{#6}%
    \ifpgfmath@in@%
      \pgf@polar@#6\@@%
    \else
      \pgf@polar@#6 and #6\@@%
    \fi
    \edef\xarcradius{\the\pgf@x}%
    \edef\yarcradius{\the\pgf@y}% 
     %
    % Get the start and end angles of the arc...
    % 
    \pgfmathsetmacro\s{#4}%
    \pgfmathsetmacro\e{#5}%
    %
    % ...and also with rounding.
    %
    \pgfmathmod@{\s}{360}%
    \ifdim\pgfmathresult pt<0pt\relax%
      \pgfmathadd@{\pgfmathresult}{360}%
    \fi
    \let\ss\pgfmathresult%
    \pgfmathmod@{\e}{360}%
    \ifdim\pgfmathresult pt<0pt\relax%
      \pgfmathadd@{\pgfmathresult}{360}%
    \fi
    \let\ee\pgfmathresult%
    %
    % Hackery for when arc straddles zero.
    %
    \ifdim\ee pt<\ss pt\relax%
      \pgfmathadd@{\x}{180}%
      \pgfmathmod@{\pgfmathresult}{360}%
      \let\x\pgfmathresult%
    \fi
    \def\m{360}% Measure of nearness.
    \pgfmathadd@{\s}{\e}%
    \pgfmathdivide@{\pgfmathresult}{2}%
    \let\n\pgfmathresult% The best estimate (default to middle of arc).
    \pgfmathloop%
      \pgfmathadd@{\s}{\e}%
      \pgfmathdivide@{\pgfmathresult}{2}%
      \let\p\pgfmathresult%
      \ifdim\p pt=\s pt\relax% 
      \else
        \tkzmathanglebetweenpoints{#2}{%
          \pgfpointadd{#3}{%
            \pgf@x\xarcradius\relax%
            \pgfmathcos@{\p}%
            \pgf@x\pgfmathresult\pgf@x%
            \pgf@y\yarcradius\relax%
            \pgfmathsin@{\p}%
            \pgf@y\pgfmathresult\pgf@y%
          }%
        }%
        %
        % Hackery for when arc straddles zero.
        %
        \ifdim\ee pt<\ss pt\relax%
          \pgfmathadd@{\pgfmathresult}{180}%
          \pgfmathmod@{\pgfmathresult}{360}%
        \fi
        \let\q\pgfmathresult%
        %
        % More hackery...
        %
        \ifdim\x pt>335pt\relax%
          \ifdim\q pt<45pt\relax%
            \pgfmathadd@{\q}{360}%
            \let\q\pgfmathresult%
          \fi
        \fi
        \ifdim\x pt=\q pt% Found it!
            \pgfmathbreakloop% Breaks after current iteration is complete.
          \else
            \ifdim\x pt<\q pt\relax%
              \let\e\p%
            \else
              \let\s\p%
            \fi
          \fi
          \pgfmathsubtract@{\x}{\q}%
          \pgfmathabs@{\pgfmathresult}%
          %
          % Save the estimate if it is better than any previous estimate.
          %
          \ifdim\pgfmathresult pt<\m pt\relax%
            \let\m\pgfmathresult%
            \let\n\p%
          \fi        
    \repeatpgfmathloop%
    \pgfpointadd{#3}{\pgfpointpolar{\n}{\xarcradius and \yarcradius}}%
  }%
}

% \tkzmathangleonellipse
% 
% Find the angle corresponding to a point on the border of an ellispe.
%
% #1 - the point on the border.
% #2 - the radii of the ellipse.
%
\def\tkzmathangleonellipse#1#2{%
  \begingroup
    \pgfmath@in@{and }{#2}%
    \ifpgfmath@in@%
      \pgf@polar@#2\@@%
    \else
      \pgf@polar@#2 and #2\@@%
    \fi
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \pgf@process{#1}% 
    \ifdim\pgf@x=0pt\relax%
      \pgfutil@tempdima1pt\relax%
    \else
      \pgfutil@tempdima\pgf@x%
%\pgfmathdivide@{\pgfmath@tonumber{\pgf@xa}}{\pgfmath@tonumber{\pgfutil@tempdima}}% 
\FPdiv\pgfmathresult{\pgfmath@tonumber{\pgf@xa}}{\pgfmath@tonumber{\pgfutil@tempdima}} 
\FPround\pgfmathresult\pgfmathresult5\relax%
      \pgfutil@tempdima\pgfmathresult pt\relax%
    \fi
    \ifdim\pgf@y=0pt\relax%
      \pgfutil@tempdima1pt\relax%
    \else 
     % \pgfmathdivide@{\pgfmath@tonumber{\pgf@y}}{\pgfmath@tonumber{\pgf@ya}}%
      \FPdiv\pgfmathresult{\pgfmath@tonumber{\pgf@y}}{%
                           \pgfmath@tonumber{\pgf@ya}}%
      \FPround\pgfmathresult\pgfmathresult5\relax%
      \pgfutil@tempdima\pgfmathresult\pgfutil@tempdima%
      \pgfmathatan@{\pgfmath@tonumber{\pgfutil@tempdima}}%
    \fi
    %
    \pgfutil@tempdima\pgfmathresult pt\relax%
    \ifdim\pgfutil@tempdima<0pt\relax%
      \advance\pgfutil@tempdima360pt\relax%
    \fi
    \ifdim\pgf@x<0pt\relax%
      \ifdim\pgf@y=0pt\relax%
        \pgfutil@tempdima180pt\relax%
      \else
        \ifdim\pgf@y<0pt\relax%
          \advance\pgfutil@tempdima180pt\relax%
        \else
          \advance\pgfutil@tempdima-180pt\relax%
        \fi
      \fi
    \else
      \ifdim\pgf@x=0pt\relax%
        \ifdim\pgf@y<0pt\relax%
          \pgfutil@tempdima270pt\relax%
        \else
          \pgfutil@tempdima90pt\relax%
        \fi
      \else
        \ifdim\pgf@y=0pt\relax%
          \pgfutil@tempdima0pt\relax%
        \fi
      \fi        
    \fi
    \pgfmath@returnone\pgfutil@tempdima%
  \endgroup
} 

\def\tkzpointborderellipse#1#2{%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \ifdim\pgf@xa=\pgf@ya% circle. that's easy!
    \pgf@process{\pgfpointnormalised{#1}}%
    \pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@x%
    \pgf@y=\pgf@sys@tonumber{\pgf@xa}\pgf@y%
  \else
    \ifdim\pgf@xa<\pgf@ya%
      % Ok, first, let's compute x/y:
      \c@pgf@countb=\pgf@ya%
      \divide\c@pgf@countb by65536\relax%
      \divide\pgf@x by\c@pgf@countb%
      \divide\pgf@y by\c@pgf@countb%
      \pgf@xc=\pgf@x%
      \pgf@yc=8192pt%
      \pgf@y=.125\pgf@y%
      \c@pgf@countb=\pgf@y%
      \divide\pgf@yc by\c@pgf@countb%
      \pgf@process{#1}%
      \pgf@y=\pgf@sys@tonumber{\pgf@yc}\pgf@y%
      \pgf@y=\pgf@sys@tonumber{\pgf@xc}\pgf@y%
      \pgf@process{\pgfpointnormalised{}}%
      \pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@x%
      \pgf@y=\pgf@sys@tonumber{\pgf@ya}\pgf@y%
    \else
      % Ok, now let's compute y/x:
      \c@pgf@countb=\pgf@xa%
      \divide\c@pgf@countb by65536\relax%
      \divide\pgf@x by\c@pgf@countb%
      \divide\pgf@y by\c@pgf@countb%
      \pgf@yc=\pgf@y%
      \pgf@xc=8192pt%
      \pgf@x=.125\pgf@x%
      \c@pgf@countb=\pgf@x%
      \divide\pgf@xc by\c@pgf@countb%
      \pgf@process{#1}%
      \pgf@x=\pgf@sys@tonumber{\pgf@yc}\pgf@x%
      \pgf@x=\pgf@sys@tonumber{\pgf@xc}\pgf@x%
      \pgf@process{\pgfpointnormalised{}}%
      \pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@x%
      \pgf@y=\pgf@sys@tonumber{\pgf@ya}\pgf@y%
    \fi  
  \fi
}    
\endinput   

==> tkz-tools-misc.tex <==
% Copyright 2011 by Alain Matthes
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.


\def\fileversion{1.16 c}
\def\filedate{2011/06/01}  


%<--------------------------------------------------------------------------–>
%                                         tkzText
%<--------------------------------------------------------------------------–>
\newif\iftkz@node\tkz@nodefalse  

\def\tkz@parsenode#1{%
\tkz@getvirg#1,\@nil
\iftkz@node  
\else
  \tkz@getfromcart#1\@nil   
\fi  
}   
\def\tkz@getvirg#1,#2\@nil{%
\ifx\tkzempty#2\tkzempty%
   \tkz@nodetrue 
\else
   \tkz@nodefalse  
\fi
}      


\def\tkzText{\pgfutil@ifnextchar[{\tkz@Text}{\tkz@Text[]}}
\def\tkz@Text[#1](#2)#3{%
 \begingroup
 \tkz@parsenode{#2} 
 \iftkz@node \node[#1] at (#2){#3}; 
 \else
 \FPadd{\ptxa}{\tkz@absc}{-\tkz@init@xorigine}
 \FPadd{\ptya}{\tkz@ord}{-\tkz@init@yorigine}
 \FPdiv{\ptxa}{\ptxa}{\tkz@init@xstep}
 \FPdiv{\ptya}{\ptya}{\tkz@init@ystep}
  \node[#1] at (\ptxa,\ptya){#3};% 
  \fi
\endgroup
}%
% %<--------------------------------------------------------------------------–>
% %                                    légende
% %<--------------------------------------------------------------------------–>
\newif\iftkz@legend@line
\pgfkeys{
/tkzlegend/.cd,  
line/.is if                 = tkz@legend@line,
line/.default               = true,
/tkzlegend/.unknown/.code   = {\let\searchname=\pgfkeyscurrentname
                              \pgfkeysalso{\searchname/.try=#1,
                                   /tikz/\searchname/.retry=#1}}  
}

\def\tkzLegend{\pgfutil@ifnextchar[{\tkz@Legend}{\tkz@Legend[]}} 
\def\tkz@Legend[#1](#2,#3)#4{%
\pgfkeys{/tkzlegend/.cd,
line=false}  
 \pgfqkeys{/tkzlegend}{#1}
 \begingroup  
\c@pgfmath@counta=0 %
\FPadd{\ptxa}{#2}{-\tkz@init@xorigine}
\FPadd{\ptya}{#3}{-\tkz@init@yorigine}
\FPdiv{\ptxa}{\ptxa}{\tkz@init@xstep}
\FPdiv{\ptya}{\ptya}{\tkz@init@ystep}
\node[/tkzlegend/.cd,#1] at (\ptxa,\ptya) {%
\begin{tikzpicture}
   \foreach \motif/\size/\col/\mtext in {#4}{%
       \iftkz@legend@line
          \draw[color      = \col,
                line width = \size,
                style      = \motif,
                text       = \tkz@mainlinecolor]%
          (0cm ,\the\c@pgfmath@counta ex)--%
               (\tkz@legend@line@len,\the\c@pgfmath@counta ex) 
       \else  
          \draw plot[mark size    = \size,%
                     mark         = \motif,%
                     mark options = {color=\col}]%
           coordinates{(0 ex,\the\c@pgfmath@counta ex)}%
         \fi
           node[right=1ex] {\mtext};
          \global\advance\c@pgfmath@counta by 3 %  
       }% 

\end{tikzpicture}%
};% 
\endgroup
}   

%<--------------------------------------------------------------------------–>
%                                 hline  pb  avec line
%<--------------------------------------------------------------------------–>
\def\tkzHLine{\pgfutil@ifnextchar[{\tkz@HLine}{\tkz@HLine[]}}  
\def\tkz@HLine[#1]#2{%
 \begingroup
    \FPeval{\tkz@valy}{(#2)}%
    \FPadd{\tkz@ptya}{\tkz@valy}{-\tkz@init@yorigine}
    \FPdiv{\tkz@ptya}{\tkz@ptya}{\tkz@init@ystep}
    \draw[#1] (\tkz@xa,\tkz@ptya)--(\tkz@xb,\tkz@ptya);%
\endgroup
}
%<--------------------------------------------------------------------------–>
%                                 hlines  pb  avec line
%<--------------------------------------------------------------------------–>
\def\tkzHLines{\pgfutil@ifnextchar[{\tkz@HLines}{\tkz@HLines[]}}  
\def\tkz@HLines[#1]#2{%
 \begingroup 
 \foreach \tkz@vy in {#2}{%
   \FPeval\my@tkz@vy{\tkz@vy}
   \tkz@HLine[#1]{\my@tkz@vy}}   
\endgroup
}  
%<--------------------------------------------------------------------------->
%                                      vline
%<--------------------------------------------------------------------------->
\def\tkzVLine{\pgfutil@ifnextchar[{\tkz@VLine}{\tkz@VLine[]}}
\def\tkz@VLine[#1]#2{%
\begingroup
  \FPeval\tkz@valx{(#2)}%
  \FPadd{\tkz@ptxa}{\tkz@valx}{-\tkz@init@xorigine}
  \FPdiv{\tkz@ptxa}{\tkz@ptxa}{\tkz@init@xstep}
  \draw[#1](\tkz@ptxa,\tkz@ya)--(\tkz@ptxa,\tkz@yb);
\endgroup
}  

%<--------------------------------------------------------------------------->
%                                      vlines
%<--------------------------------------------------------------------------->
\def\tkzVLines{\pgfutil@ifnextchar[{\tkz@VLines}{\tkz@VLines[]}}
\def\tkz@VLines[#1]#2{%
\begingroup  
 \foreach \tkz@vx in {#2}{%  
   \FPeval\my@tkz@vx{\tkz@vx}
   \tkz@VLine[#1]{\my@tkz@vx}}  
\endgroup
} 
%<--------------------------------------------------------------------------–>
\def\tkzHTick{\pgfutil@ifnextchar[{\tkz@HTick}{\tkz@HTick[]}}  
\def\tkz@HTick[#1]#2{%
 \begingroup  
    \FPeval\tkz@ptxa{(#2)}% 
    \FPround\tkz@ptxa\tkz@ptxa{5}   
    \FPclip\tkz@ptxa\tkz@ptxa
    \FPadd\tkz@ptxa\tkz@ptxa{-\tkz@init@xorigine}
    \FPdiv\tkz@ptxa\tkz@ptxa{\tkz@init@xstep} 
    \draw plot[mark style,#1] coordinates {(\tkz@ptxa,0)};  
\endgroup
}
\def\tkzHTicks{\pgfutil@ifnextchar[{\tkz@HTicks}{\tkz@HTicks[]}}  
\def\tkz@HTicks[#1]#2{%
 \begingroup 
\foreach \tkz@hy in {#2} {\tkz@HTick[#1]{\tkz@hy}}
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzVTick{\pgfutil@ifnextchar[{\tkz@VTick}{\tkz@VTick[]}}  
\def\tkz@VTick[#1]#2{%
 \begingroup
    \FPeval\tkz@ptya{(#2)}%
    \FPround\tkz@ptya\tkz@ptya{5}%
    \FPclip\tkz@ptya\tkz@ptya
    \FPadd\tkz@ptya\tkz@ptya{-\tkz@init@yorigine}%
    \FPdiv\tkz@ptya\tkz@ptya{\tkz@init@ystep}%
    \draw plot[mark style,#1] coordinates {(0,\tkz@ptya)};
\endgroup
}
%<--------------------------------------------------------------------------–>
\def\tkzVTicks{\pgfutil@ifnextchar[{\tkz@VTicks}{\tkz@VTicks[]}}  
\def\tkz@VTicks[#1]#2{%
\begingroup 
\foreach \tkz@hy in {#2} {\tkz@VTick[#1]{\tkz@hy}}
\endgroup
} 
\endinput

==> tkz-tools-obsolete.tex <==
\makeatletter
\global\edef\tkz@sua@lw{0.4pt} 
\global\edef\tkz@sua@color{black} 
\global\edef\tkz@sua@gradsize{\textstyle} 
\global\edef\tkz@sua@tickwd{0.8 pt}
\global\edef\tkz@sua@ticka{2 pt}  
\global\edef\tkz@sua@tickb{2 pt}



\def\tkzX{\pgfutil@ifnextchar[{\tkz@X}{\tkz@X[]}}
\def\tkz@X[#1]{% 
\begingroup
 \pgfkeys{/tkzX/.cd,
 trig     = 0,
 lw       = \tkz@sua@lw,
 gradsize = \tkz@sua@gradsize,
 color    = \tkz@sua@color,
 tickwd   = \tkz@sua@tickwd,
 tickup   = \tkz@sua@ticka,
 tickdn   = \tkz@sua@tickb,  
 pos      = {below = 3pt},
 label    = $x$,
 poslabel = {below = 3pt},
 noticks  = false,
 nograd   = false,
% unit     = false,
 orig     = false,
 step    = \tkz@init@xstep
 }    
 \pgfqkeys{/tkzX}{#1}  
   \FPtrunc\posmax{\tkz@xb}{\tkz@init@xdec}%
   \FPtrunc\posmin{\tkz@xa}{\tkz@init@xdec}%
   \FPdiv\tkz@posnext{\tkz@posnext}{\tkz@init@xstep}
   \FPadd\posnext{\posmin}{\tkz@posnext}
   \FPadd\tkz@xbsup{\tkz@xb}{\tkz@init@rightspace}
   \path (\tkz@xa,0)--(\tkz@xb,0) node(tkz@xline){};%
    \protected@edef\tkz@temp{%
    \noexpand%    
   \draw[xaxe style,line width = \tkz@X@lw,%
         color      = \tkz@X@color]%
        (\tkz@xa,0)--(\tkz@xbsup,0)%
         node[xlabel style,\tkz@X@poslabel]}\tkz@temp%
         {\tkz@X@label};%
    \FPtrunc\xtkzero{0.0000000}{\tkz@init@xdec}% 
   \iftkz@X@noticks%
   \else 
\ifnum\tkz@X@trig=0%
   \FPtrunc\posmax{\posmax}{\tkz@init@xdec}% 
   \foreach \pos in {\posmin,\posnext,...,\posmax}{%
      \FPtrunc\tkz@pos{\pos}{\tkz@init@xdec}%
      \protected@edef\tkz@temp{%
      \noexpand% 
       \draw[line width = \tkz@X@tickwd,shift = {(\pos,0)}]%
            (0pt,\tkz@X@tickup)--(0pt,-\tkz@X@tickdn)%
            node[\tkz@X@pos,inner sep = 0pt]}\tkz@temp
        {\FPmul{\xgrad}{\pos}{\tkz@init@xstep}%
         \FPadd{\xgrad}{\xgrad}{\tkz@init@xorigine}%
         \FPtrunc\xgrad{\xgrad}{\tkz@init@xdec}%
         \iftkz@X@orig% 
               \iftkz@X@nograd
               \else\tkz@showgrad{\xgrad}%
                  $\textcolor{\tkz@sur@colorlabel}{%
                  \tkz@X@gradsize{\numprint{\tkz@result}}}$%
               \fi
          \else % orig
            \iftkz@init@NO% 
               \ifx\tkz@pos\posmin
               \else
                  \tkz@showgrad{\xgrad}%
                  $\textcolor{\tkz@sur@colorlabel}{%
                  \tkz@X@gradsize{\numprint{\tkz@result}}}$
               \fi
            \else % NO
               \ifx\tkz@pos\xtkzero%
                   % \iftkz@X@unit\tkz@showgrad{\xgrad}%
                   % $\textcolor{\tkz@sur@colorlabel}{%
                   % \tkz@X@gradsize{\numprint{\tkz@result}}}$
                   % \fi  
               \else 
                  \iftkz@X@nograd%
                  \else\tkz@showgrad{\xgrad}%
                    $\textcolor{\tkz@sur@colorlabel}{%
                     \tkz@X@gradsize{\numprint{\tkz@result}}}$
                  \fi
               \fi%end of xtkzero
          \fi%end of NO
      \fi%end of orig
};%  end of draw
}% end foreach
   \else %trig affichage
       \FPadd{\posmin}{\posmin}{0.5}%
       \FPdiv\nbtrigticksmax{\posmax}{\FPpi}%
       \FPdiv\nbtrigticksmin{\posmin}{\FPpi}%
       \FPmul\nbtrigticksmax{\nbtrigticksmax}{\tkz@X@trig}%
       \FPmul\nbtrigticksmin{\nbtrigticksmin}{\tkz@X@trig}%
       \FPround\nbtrigticksmin{\nbtrigticksmin}{0}% 
       \foreach \pos in {\nbtrigticksmin,...,\nbtrigticksmax}{%
          \FPmul\pospi{\pos}{\FPpi}
          \FPdiv\pospi{\pospi}{\tkz@X@trig}%
          \protected@edef\tkz@temp{%
          \noexpand\draw[line width = \tkz@X@tickwd,%
                         shift      = {(\pospi,0)}]%
                      (0pt,\tkz@X@tickup)--(0pt,-\tkz@X@tickup)%
                      node[\tkz@X@pos,%
                           text height = 8pt,%
                           inner sep   = 1pt]}\tkz@temp%
                {\tkzPrintFracWithPi{\pos}{\tkz@X@trig}%
                 \tkzprintfrac};% 
        }% end foreach                              
    \fi
\fi% end ticks  
\endgroup
 }% todo macro pour l'affichage 

%<--------------------------------------------------------------------------–>
%                                 tkzY
%<--------------------------------------------------------------------------–>

\pgfkeys{
  tkzY/.cd,
  pos/.code        = {\def\tkz@Y@pos{#1}},
  trig/.code       = {\def\tkz@Y@trig{#1}},
  lw/.code         = {\def\tkz@Y@lw{#1}},
  color/.code      = {\def\tkz@Y@color{#1}},
  label/.code      = {\def\tkz@Y@label{#1}},  
  poslabel/.code   = {\def\tkz@Y@poslabel{#1}},
  tickwd/.code     = {\def\tkz@Y@tickwd{#1}},
  ticklt/.code     = {\def\tkz@Y@ticklt{#1}},
  tickrt/.code     = {\def\tkz@Y@tickrt{#1}},
  gradsize/.code   = {\def\tkz@Y@gradsize{#1}},
  step/.code       = {\def\tkz@posnext{#1}}, 
  noticks/.is if   = tkz@Y@noticks,
  noticks/.default = true,  
  nograd/.is if    = tkz@Y@nograd,
  nograd/.default  = true,  
  orig/.is if      = tkz@Y@orig,
  orig/.default    = true,  
  unit/.is if      = tkz@Y@unit,
  unit/.default    = true  }    
\def\tkzY{\pgfutil@ifnextchar[{\tkz@Y}{\tkz@Y[]}}
\def\tkz@Y[#1]{%
 \pgfkeys{/tkzY/.cd,
 trig     = 0,
 lw       = \tkz@sua@lw,
 gradsize = \tkz@sua@gradsize,
 color    = \tkz@sua@color,
 tickwd   = \tkz@sua@tickwd,
 tickrt   = \tkz@sua@ticka,
 ticklt   = \tkz@sua@tickb,
 label    = $y$,
 poslabel = {left = 3pt},
 pos      = {left = 3pt},   
 noticks  = false,
 nograd   = false,
 unit     = false,
 orig     = false,
 step     = \tkz@init@ystep
 }    
 \pgfqkeys{/tkzY}{#1}  
   \FPtrunc\posmax{\tkz@yb}{\tkz@init@ydec}%
   \FPtrunc\posmin{\tkz@ya}{\tkz@init@ydec}%
     \FPdiv\tkz@posnext{\tkz@posnext}{\tkz@init@ystep}
   \FPadd\posnext{\posmin}{\tkz@posnext}  
   \path (0,\tkz@ya)--(0,\tkz@yb) node(tkz@yline){};%
   \FPadd\tkz@ybsup{\tkz@yb}{\tkz@init@upspace}   
   \protected@edef\tkz@temp{%
   \noexpand% 
   \draw[line width = \tkz@Y@lw,%
         color      = \tkz@Y@color,yaxe style]%
        (0,\tkz@ya)--(0,\tkz@ybsup)%
        node[\tkz@Y@poslabel,ylabel style]}\tkz@temp%
        {\tkz@Y@label};%
   \FPtrunc\ytkzero{0.000000}{\tkz@init@ydec}%
   \iftkz@Y@noticks%
   \else
   \foreach \pos in {\posmin,\posnext,...,\posmax}{%
       \FPtrunc\tkz@pos{\pos}{\tkz@init@ydec}%
       \protected@edef\tkz@temp{%
       \noexpand% 
       \draw[line width = \tkz@Y@tickwd,%
            shift       = {(0,\pos)}]%
            (\tkz@Y@tickrt,0pt)--(-\tkz@Y@ticklt,0pt)%
            node[\tkz@Y@pos,inner sep = 0pt]}\tkz@temp%
         {\FPmul{\ygrad}{\pos}{\tkz@init@ystep}%
          \FPadd{\ygrad}{\ygrad}{\tkz@init@yorigine}
          \FPtrunc\ygrad{\ygrad}{\tkz@init@ydec}%
          \iftkz@Y@orig% 
              \iftkz@Y@nograd\else\tkz@showgrad{\ygrad}%
                         $\textcolor{\tkz@sur@colorlabel}{\tkz@Y@gradsize{\numprint{\tkz@result}}}$\fi
          \else
           \iftkz@init@NO% 
             \ifx\tkz@pos \posmin\else
             \tkz@showgrad{\ygrad}%
                 $\textcolor{\tkz@sur@colorlabel}{\tkz@Y@gradsize{\numprint{\tkz@result}}}$\fi
        \else 
          \ifx\tkz@pos \ytkzero 
            \iftkz@Y@unit\tkz@showgrad{\ygrad}%
               $\textcolor{\tkz@sur@colorlabel}{\tkz@Y@gradsize{\numprint{\tkz@result}}}$\fi\else
            \iftkz@Y@nograd%
             \else \tkz@showgrad{\ygrad}%
              $\textcolor{\tkz@sur@colorlabel}{\tkz@Y@gradsize{\numprint{\tkz@result}}}$\fi\fi
        \fi
    \fi
   };%
  }%
\fi
\iftkz@init@NO\else\iftkz@Y@unit%
  \draw[line width = 1pt,%
        inner sep  = 1pt] (0,0) -- (0,1)%
        node[left=3pt]%
       {$\tkz@Y@gradsize{\numprint{\tkz@init@ystep}}$};% 
  \draw[line width = \tkz@Y@tickwd,%
        shift      = {(0,1)}]%
      (\tkz@Y@tickrt,0pt)--(-\tkz@Y@ticklt,0pt);%
  \fi\fi
}%
\makeatother
\endinput 

==> tkz-tools-utilities.tex <==
% Copyright 2011 by Alain Matthes
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.


\def\fileversion{1.16 c}
\def\filedate{2011/06/01}

%<--------------------------------------------------------------------------–>
\def\tkzutil@empty{}
\def\tkzutil@firstofone#1{#1}
\def\tkzutil@firstoftwo#1#2{#1}
\def\tkzutil@secondoftwo#1#2{#2}
%<--------------------------------------------------------------------------–>
\long\def\tkzutil@ifundefined#1{%
  \expandafter\ifx\csname#1\endcsname\relax
    \expandafter\tkzutil@firstoftwo
  \else
    \expandafter\tkzutil@secondoftwo
  \fi} 
%<--------------------------------------------------------------------------–>
%<--------------------------------------------------------------------------–>
\global\def\tkzActivOff{%
\edef\tkzTwoPtCode{\the\catcode`\:} 
\edef\tkzPtExCode{\the\catcode`\!} 
\edef\tkzPtVirCode{\the\catcode`\;} 
\catcode`\:=12 \catcode`\!=12 \catcode`\;=12}%
\global\def\tkzActivOn{%
\catcode`\:=\tkzTwoPtCode\relax
\catcode`\!=\tkzPtExCode\relax
\catcode`\;=\tkzPtVirCode\relax
}% 
 
%<----------------------------– autres tools -------------------------------->   
%<--------------------------  Initialisation -------------------------------->   
\pgfkeys{
/tkzsupcol/.cd,
  background/.code    = {\global\edef\tkz@suc@bkc{#1}},%
  text/.code          = {\global\edef\tkz@suc@txt{#1}}, 
} 
\def\tkzSetUpColors{\pgfutil@ifnextchar[{\tkz@SetUpColors}{\tkz@SetUpColors[]}} 
\def\tkz@SetUpColors[#1]{%
\begingroup
\pgfkeys{%
tkzsupcol/.cd,
  background  = \tkz@backgroundcolor,
  text        = \tkz@textcolor
  }
\pgfqkeys{/tkzsupcol}{#1} 
\global\edef\tkz@fillcolor{\tkz@suc@bkc}   
\global\edef\tkz@mainlinecolor{\tkz@suc@txt}
\global\edef\tkz@textcolor{\tkz@suc@txt}
\global\def\tkz@otherlinecolor{\tkz@suc@txt!50}
\global\edef\tkz@sua@color{\tkz@mainlinecolor}       
\pagecolor{\tkz@suc@bkc}
\color{\tkz@suc@txt}  
 \InputIfFileExists{tkz-base.cfg}{\typeout{Local configuration file tkz-param.cfg found and used}}{\typeout{tkz-base.cfg not found}  
%<---------   axes cartesian system  ---------------------------------------–>  
\global\edef\tkz@init@color{\tkz@textcolor} 
\global\def\tkz@init@lw{0.4 pt}
\global\def\tkz@init@xlabel{$x$}
\global\def\tkz@init@ylabel{$y$}  
\global\def\tkz@init@tickwd{0.8 pt}
\global\def\tkz@init@ticka{2 pt}  
\global\def\tkz@init@tickb{2 pt}
\global\def\tkz@init@rightspace{.5} 
\global\def\tkz@init@leftspace{0}
\global\def\tkz@init@upspace{.5} 
\global\def\tkz@init@downspace{0}
\global\let\tkzmathstyle\displaystyle   
\tikzset{xlabel style/.style={below=3 pt,
                              inner sep = 1pt,
                              outer sep = 0pt}}
\tikzset{xaxe style/.style ={>=latex,->}}
\tikzset{ylabel style/.style={left = 3 pt,
                              inner sep = 1pt,
                              outer sep = 0pt}}
\tikzset{yaxe style/.style ={>=latex,->}} 
%<--------------------------   rep  ---------------------------------------–>
\global\edef\tkz@sur@color{\tkz@mainlinecolor}
\global\edef\tkz@sur@colorlabel{\tkz@mainlinecolor}
\global\def\tkz@sur@lw{0.8 pt}
\global\def\tkz@sur@posxlabel{below=2pt}
\global\def\tkz@sur@posylabel{left=2pt} 
%<--------------------------   grid  ---------------------------------------–>
\global\edef\tkz@grid@color{gray}
\global\def\tkz@grid@lw{0.4 pt}
\global\def\tkzCoeffSubColor{50} 
\global\def\tkzCoeffSubLw{0.8}
\global\def\tkz@grid@xstep{0.2}
\global\def\tkz@grid@ystep{0.2}  
%<--------------------------   line  ---------------------------------------–>
\global\edef\tkz@euc@linecolor{\tkz@mainlinecolor}
\global\def\tkz@euc@linewidth{0.6pt}
\global\def\tkz@euc@linestyle{solid}
\global\def\tkz@euc@lineleft{.2}
\global\def\tkz@euc@lineright{.2}
\global\def\tkz@legend@line@len{1cm}  
\global\edef\tkz@euc@segmentcolor{\tkz@mainlinecolor}
\global\edef\tkz@euc@circlecolor{\tkz@mainlinecolor}
\tikzset{line style/.style={%
         line width = \tkz@euc@linewidth,
         color      = \tkz@euc@linecolor,
         style      = \tkz@euc@linestyle,
         add        = {\tkz@euc@lineleft} and {\tkz@euc@lineright}}}  
%<--------------------------    points   -----------------------------------–>
\global\edef\tkz@euc@pointshape{circle}
\global\edef\tkz@euc@pointcolor{\tkz@mainlinecolor}
\global\edef\tkz@euc@labelcolor{\tkz@mainlinecolor} 
\global\def\tkz@euc@pointsize{6}
\global\def\tkz@euc@pointpos{below right}
\tikzset{point style/.style={draw         = \tkz@euc@pointcolor,
                             inner sep    = 0pt,
                             shape        = \tkz@euc@pointshape,
                             minimum size = \tkz@euc@pointsize*\pgflinewidth,
                             fill         = \tkz@euc@pointcolor!50}}  
%<----------------------------    mark   -----------------------------------–> 
\global\edef\tkz@mk@color{\tkz@mainlinecolor}   
\global\edef\tkz@mk@mark{*}
\global\edef\tkz@mk@size{3pt}
\global\edef\tkz@mk@fill{\tkz@otherlinecolor} 
\tikzset{mark style/.style={mark=\tkz@mk@mark,mark size=\tkz@mk@size,mark options={color=\tkz@mk@color,fill=\tkz@mk@fill}}}
\tikzset{arrow coord style/.style={dashed,
                             \tkz@euc@linecolor,
                             >=latex',
                             ->}}
\tikzset{xcoord style/.style={\tkz@euc@labelcolor,
                           font=\normalsize,text height=1ex,
                           inner sep = 0pt,
                           outer sep = 0pt,
                           fill=\tkz@fillcolor,
                           below=3pt}} 
\tikzset{ycoord style/.style={\tkz@euc@labelcolor,
                           font=\normalsize,text height=1ex, 
                           inner sep = 0pt,
                           outer sep = 0pt, 
                           fill=\tkz@fillcolor,
                           left=3pt}}  
%<---------------------------  vector --------------------------------------–>
\tikzset{vector style/.style={>=latex,->}}   
%<-------------------------    compass   -----------------------------------–> 
\global\edef\tkz@euc@compasscolor{\tkz@otherlinecolor}
\global\def\tkz@euc@compasswidth{0.4pt}
\global\def\tkz@euc@compassstyle{solid}  
\tikzset{compass style/.style={color      = \tkz@euc@compasscolor,
                               line width = \tkz@euc@compasswidth,
                               style      = \tkz@euc@compassstyle}}    
}
\endgroup}

%<--------------------------------------------------------------------------–>
%              Pour savoir le nombre de décimales d'un nombre
% le nombre dans #1 et le résultat dans \c@pgfmath@countb
%<--------------------------------------------------------------------------–>

\newcommand*\tkz@getdecimal[1]{%
  \expandafter\@getdecimal#1.\@nil
}

\def\@getdecimal#1.#2\@nil{%
  \ifx\empty#2\empty
    % Si #2 est vide, c'est qu'il n'y avait pas de point
    % dans la chaîne initiale
    \c@pgfmath@countb0 %
   \global\def\tkz@decpart{}%
  \else
    % sinon c'est la chaîne qui suit le point décimal...
    \CountToken{#2}%
    % ... y compris le point en trop ajouté par \tkz@getdecimal  :-)
    \advance\c@pgfmath@countb by-1 %
    \@@getdecimal#2\@nil
  \fi
}
\def\@@getdecimal#1.\@nil{\global\def\tkz@decpart{#1}}
%<--------------------------------------------------------------------------–>
% code from JCC modifi
\newcommand\CountToken[1]{%
 \c@pgfmath@countb0 %
  \expandafter\C@untToken#1\@nil
%modifi ajout du expandafter
}
\newcommand\C@untToken{%
  \afterassignment\C@untT@ken\let\CurrT@ken=
}
\newcommand\C@untT@ken{%
 \ifx\CurrT@ken\@nil \else
   \advance\c@pgfmath@countb by1 %
   \expandafter\C@untToken
 \fi
}
% end code from JCC    

%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%            Tools
%<–––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––––>
%<–––––––– code from TeX in Practice ––––––––>
\newif\if@TestSubString
\def\SubStringConditional #1#2{%
    TT\fi
    \edef\@MainString{#1}%
    \edef\@SubStringConditionalTemp{{#1}{#2}}%
    \expandafter\@SubStringConditional\@SubStringConditionalTemp
}
\def\@SubStringConditional #1#2{% 
    \def\@TestSubS ##1#2##2\\{% 
        \def\@TestTemp{##1}% 
    }% 
    \@TestSubS #1#2\\
    \ifx\@MainString\@TestTemp
        \@TestSubStringfalse
    \else
        \@TestSubStringtrue
    \fi
    \if@TestSubString
}

\def\RecursionMacroEnd #1#2#3{% 
    #1\relax
        \def\@RecursionMacroEndNext{#2}% 
    \else
        \def\@RecursionMacroEndNext{#3}% 
    \fi
    \@RecursionMacroEndNext
}

\def\ReplaceSubStrings #1#2#3#4{%
    \def\@ReplaceResult{#1}%
    \edef\@ReplaceMain{#2}%
    \edef\@ReplaceSub{#3}%
    \edef\@ReplaceSubRep{#4}%
    \@ReplaceSubStrings
}
\def\@ReplaceSubStrings{% 
    \RecursionMacroEnd
        {\if\SubStringConditional{\@ReplaceMain}{\@ReplaceSub}}%
      {\@ReplaceSubStringsDo}{\expandafter\edef\@ReplaceResult{\@ReplaceMain}}%
}
\def\@ReplaceSubStringsDoX{%
    \def\@ReplaceSubStringsDoA ##1%
}%
\def\@ReplaceSubStringsDo{% 
    \expandafter\@ReplaceSubStringsDoX \@ReplaceSub
                                    ##2\@EndReplaceSubStrings{%
        \edef\@ReplaceMain{##1\@ReplaceSubRep ##2}%
    }%
    \expandafter\@ReplaceSubStringsDoA\@ReplaceMain
        \@EndReplaceSubStrings
    \@ReplaceSubStrings
}
\def\tkzPrintFrac#1#2{% 
\begingroup
\tkzReducFrac{#1}{#2}
\global\edef\tkzprintfrac{$     \frac{\tkzMathFirstResult}{\tkzMathSecondResult}$}%
 \ifnum\tkzMathFirstResult=0%
    \global\edef\tkzprintfrac{$0$}%
 \else
 \ifnum\tkzMathSecondResult=1 %
    \ifnum\tkzMathFirstResult=1 %
         \global\edef\tkzprintfrac{$1$}%
      \else
       \ifnum\tkzMathFirstResult=-1%
          \global\edef\tkzprintfrac{$-1$}%
        \else
          \global\edef\tkzprintfrac{$\tkzMathFirstResult$}%
       \fi\fi
 \else 
   \ifnum\tkzMathFirstResult=1 %
          \global\edef\tkzprintfrac{$\tkzmathstyle\frac{1}{\tkzMathSecondResult}$}%
     \else
       \ifnum\tkzMathFirstResult=-1 %
      \global\edef\tkzprintfrac{$\tkzmathstyle\frac{-1}{\tkzMathSecondResult}$}%
        \else
     \global\edef\tkzprintfrac{$\tkzmathstyle\frac{\tkzMathFirstResult}{%
                             \tkzMathSecondResult}$}%
 \fi\fi\fi\fi   
\endgroup}
%<--------------------------------------------------------------------------->
\def\tkzPrintFracWithPi#1#2{% 
\begingroup
\tkzReducFrac{#1}{#2}
\global\edef\tkzprintfrac{$\tkzmathstyle\frac{\tkzMathFirstResult\pi}{\tkzMathSecondResult}$}%
 \ifnum\tkzMathFirstResult=0%
    \global\edef\tkzprintfrac{$0$}%
 \else
 \ifnum\tkzMathSecondResult=1 %
    \ifnum\tkzMathFirstResult=1 %
         \global\edef\tkzprintfrac{$\pi$}%
      \else
       \ifnum\tkzMathFirstResult=-1%
          \global\edef\tkzprintfrac{$-\pi$}%
        \else
          \global\edef\tkzprintfrac{$\tkzMathFirstResult\pi$}%
       \fi\fi
 \else 
   \ifnum\tkzMathFirstResult=1 %
          \global\edef\tkzprintfrac{$\tkzmathstyle\frac{\pi}{\tkzMathSecondResult}$}%
     \else
       \ifnum\tkzMathFirstResult=-1 %
      \global\edef\tkzprintfrac{$\tkzmathstyle\frac{-\pi}{\tkzMathSecondResult}$}%
        \else
     \global\edef\tkzprintfrac{$\tkzmathstyle\frac{\tkzMathFirstResult\pi}{%
                             \tkzMathSecondResult}$}%
 \fi\fi\fi\fi   
\endgroup}%

%<--------------------------------------------------------------------------->
% chargement des modules
\def\tkz@obj@all{polygons,vectors,arcs,sectors,angles,protractor}
\def\tkz@obj@txt{all}
\def\usetkzobj{\pgfutil@ifnextchar[{\use@usetkzobj}{\use@@usetkzobj}}%}
\def\use@usetkzobj[#1]{\use@@usetkzobj{#1}}
\def\use@@usetkzobj#1{% 
  \def\tkz@list{#1}
  \ifx\tkz@obj@txt\tkz@list \edef\tkz@list{\tkz@obj@all}% 
      \else  
      \edef\tkz@list{#1}%
    \fi
  %\edef\tkz@list{#1}%
  \pgfutil@for\tkz@temp:=\tkz@list\do{%
    \expandafter\ifx\csname tkz@library@\tkz@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let\csname tkz@library@\tkz@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tkz@obj@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tkz@obj@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12   
      \input tkz-obj-\tkz@temp.tex 
            \catcode`\@=\csname tkz@obj@#1@atcode\endcsname
      \catcode`\|=\csname tkz@obj@#1@barcode\endcsname  
    \fi%
  }%
}%
\def\DisabledNumprint{\let\tkz@numprint\numprint
\let\numprint\relax}
\def\EnabledNumprint{\let\numprint\tkz@numprint} 
\endinput
